SPEED: A Scalable RISC-V Vector Processor Enabling Efficient Multi-Precision DNN Inference

Deploying deep neural networks (DNNs) on those resource-constrained edge platforms is hindered by their substantial computation and storage demands. Quantized multi-precision DNNs, denoted as MP-DNNs, offer a promising solution for these limitations but pose challenges for existing RISC-V processors due to complex instructions, suboptimal parallel processing, and inefficient dataflow mapping. To tackle the challenges mentioned above, SPEED, a scalable RISC-V vector (RVV) processor, is proposed to enable efficient MP-DNN inference, incorporating innovations in customized instructions, hardware architecture, and dataflow mapping. Firstly, some dedicated customized RISC-V instructions are introduced based on RVV extensions to reduce the instruction complexity, allowing SPEED to support processing precision ranging from 4-bit to 16-bit with minimized hardware overhead. Secondly, a parameterized multi-precision tensor unit is developed and integrated within the scalable module to enhance parallel processing capability by providing reconfigurable parallelism that matches the computation patterns of diverse MP-DNNs. Finally, a flexible mixed dataflow method is adopted to improve computational and energy efficiency according to the computing patterns of different DNN operators. The synthesis of SPEED is conducted on TSMC 28nm technology. Experimental results show that SPEED achieves a peak throughput of 737.9 GOPS and an energy efficiency of 1383.4 GOPS/W for 4-bit operators. Furthermore, SPEED exhibits superior area efficiency compared to prior RVV processors, with enhancements of 5.9$\sim$26.9$\times$ and 8.2$\sim$18.5$\times$ for 8-bit operator and best integer performance, respectively, which highlights SPEED's significant potential for efficient MP-DNN inference.

==> 0-abstr.tex <==
\begin{abstract}
% Prof. Jun Lin, YYDS!
\pdfoutput=1

% Computationally intensive algorithms such as Deep Neural Networks (DNNs) have grown more complex in structure and exploded in parameters, resulting in enhanced performance. 
RISC-V processors are emerging as a promising choice in areas ranging from energy-efficient embedded systems to high-performance computing environments, thanks to the adaptation of the open-source RISC-V instruction set architecture (ISA).
On these RISC-V hardware platform, DNNs demonstrate significant deployment demands across various applications.
In contrast to DNNs, multi-precision quantized DNNs are increasingly favored for efficient deployment, reducing resource usage and improving inference speed. 
However, deploying multi-precision quantized DNNs on prior RISC-V processors poses significant challenges.

% However, this advancement poses significant deployment challenges in relation to memory limitations and computational throughput. 
% From an algorithmic perspective, employing a hybrid low-precision computation technique has proven to be a promising approach in tackling these challenges. 
% Nevertheless, some existing research falls short in supporting the computation of low-precision DNNs, while others overlook the crucial aspect of achieving a balanced trade-off between data utilisation and computational throughput.
% We present SPEED, a configurable RISC-V vector processor capable of performing multi-precision calculations in 4/8/16 bits, which is embedded a systolic array unit in expandable lanes.
% And we design a custom instruction set to control the systolic array unit, devise mixed dataflow strategy to accommodate computations involving various layer types in DNNs.
The processor, implemented using 28nm CMOS technology, achieves a peak integer performance of 172.45 GOPS at 4-bit.
Furthermore, SPEED achieves an average performance which is 6.8 times and 15.7 times better than Ara with 16-bit and 8-bit for benchmarked DNNs, respectively.
% , when accelerating the computation of Conv2d over various ranges of inputs and kernel sizes.

\end{abstract}

==> 0-bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.2in,clip,keepaspectratio]{figures/TVLSI-bio-cnwang.jpg}}]{Chuanning Wang}
received the B.E. degree in the School of Microelectronics from Tianjin University, Tianjin, China, in 2021. She is currently pursuing a Ph.D. degree in Information and Communication Engineering at Nanjing University, Nanjing, China.

Her current research interests focus on RISC-V processor design for deep neural networks (DNNs), especially RISC-V vector processor architectures.
\vspace{-0.4in}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.2in,clip,keepaspectratio]{figures/TVLSI-bio-cfang.pdf}}]{Chao Fang}
received the B.E. degree in the School of Precision Instrument and Opto-electronics Engineering from Tianjin University, Tianjin, China, in 2019. He is currently pursuing a Ph.D. degree in Information and Communication Engineering at Nanjing University, Nanjing, China.

His current research interests focus on algorithm-hardware co-optimization for deep neural networks (DNNs), especially involving exploiting efficient algorithms and architectures for DNNs, and integrating DNN accelerators with RISC-V processors.
\vspace{-0.4in}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.2in,clip,keepaspectratio]{figures/TVLSI-bio-xiaow.png}}]{Xiao Wu} received the B.S. degree in microelectronics science and engineering from Jilin University, Changchun, China, in 2019, and the Ph.D. degree in information and communication engineering from Nanjing University, Nanjing, China, in 2024.

Since August 2024, she has been a Senior Chip Research and Development Engineer with Xiaomi Inc., Shanghai. 
Her research interests focus on efficient hardware design for deep learning, especially deep neural networks (DNNs) accelerators and their performance modeling.
%very large scale integration design and deep learning, especially its hardware acceleration.
\vspace{-0.4in}
\end{IEEEbiography}



% insert where needed to balance the two columns on the last page with
% biographies
%\newpage


\begin{IEEEbiography}[{\includegraphics[width=1.25in,height=1.25in,clip,keepaspectratio]{figures/TVLSI-bio-zfwang.jpg}}]{Zhongfeng Wang}
(M'00-SM'05-F'16) received both the B.E. and M.S. degrees in the Dept. of Automation at Tsinghua University, Beijing, China, in 1988 and 1990, respectively. He obtained the Ph.D. degree from the University of Minnesota, Minneapolis, in 2000. He has been working for Nanjing University, China, as a Distinguished Professor since 2016. Previously he worked for Broadcom Corporation, California, from 2007 to 2016 as a leading VLSI architect. Before that, he worked for Oregon State University and National Semiconductor Corporation.

Dr. Wang is a world-recognized expert on Low-Power High-Speed VLSI Design for Signal Processing Systems. He has published over 200 technical papers with multiple best paper awards received from the IEEE technical societies, among which is the VLSI Transactions Best Paper Award of 2007. He has edited one book VLSI and held more than 20 U.S. and China patents. In the current record, he has had many papers ranking among top 25 most (annually) downloaded manuscripts in IEEE Trans. on VLSI Systems. In the past, he has served as Associate Editor for IEEE Trans. on TCAS-I, T-CAS-II, and T-VLSI for many terms. He has also served as TPC member and various chairs for tens of international conferences. Moreover, he has contributed significantly to the industrial standards. So far, his technical proposals have been adopted by more than fifteen international networking standards. In 2015, he was elevated to the Fellow of IEEE for contributions to VLSI design and implementation of FEC coding. His current research interests are in the area of Optimized VLSI Design for Digital Communications and Deep Learning.
\end{IEEEbiography}


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.2in,clip,keepaspectratio]{figures/TVLSI-bio-jlin.pdf}}]{Jun Lin} 
(S’14-SM’18) received the B.S. degree
in physics and the M.S. degree in microelectronics from Nanjing University, Nanjing, China, in 2007 and 2010, respectively, and the Ph.D. degree in electrical engineering from the Lehigh University, Bethlehem, in 2015. From 2010 to 2011, he was an ASIC design engineer with AMD. During summer 2013, he was an intern with Qualcomm Research, Bridgewater, NJ. In June 2015, he joined the school of electronic science and engineering of Nanjing University, where he is an associate professor. He is a member of the Design and Implementation of Signal Processing Systems (DISPS) Technical Committee of the IEEE Signal Processing Society.

His current research interests include low-power high-speed VLSI design, specifically VLSI design for digital signal processing and deep learning. He was a co-recipient of the Merit Student Paper Award at the IEEE Asia Pacific Conference on Circuits and Systems in 2008, the Best Paper Award of ISVLSI 2019. He was a recipient of the 2014 IEEE Circuits \& Systems Society (CAS) student travel award.
\vspace{-0.4in}
\end{IEEEbiography}
    

==> 1-intro.tex <==
\section{Introduction} \label{sec:intro}
%现如今DNN应用广泛，但随着性能越好越复杂参数越多
%Vec-p是一种适合处理DNN数据的好方法
%相较于DNN而言，QNN是一种适于部署的算法
%而Vec-p现有的一些工作不支持QNN的低精度数据，能够支持的数据吞吐量又小
%因此我们提出了SPEED，更适用于处理QNN的vec-p
%三个contrib如下：
%定制指令集设计
%硬件上加入了脉动阵列
%设计了更适合处理conv2d的数据流
% \par
% \vspace{1em}
% Deep neural networks (DNNs) \cite{Schmidhuber2014DeepLI} have exhibited notable achievements across a multitude of domains, including computer vision \cite{Ren2015FasterRT, Bochkovskiy2020YOLOv4OS}, speech recognition \cite{Chan2016ListenAA, Han2020ContextNetIC}, and natural language processing \cite{Raffel2019ExploringTL, Clark2020ELECTRAPT}. 
% Nevertheless, the extensive computational and memory necessities of DNNs may constrain their utilization on devices with restricted resources, such as mobile phones and Internet of Things (IoT) devices. 
% To address this challenge, low-bit DNNs \cite{Carmichael2018DeepPA, Xu2021MixedPD, Hanif2022CoNLoCNNEC} have emerged as a promising solution in recent years, attributed to their reduced memory and computation requirements and their potential for deployment on resource-constrained devices.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  wangshifu's new draft  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Deep neural networks (DNNs) have made significant achievements in various domains of machine learning such as including computer vision \cite{Ren2015FasterRT, Bochkovskiy2020YOLOv4OS}, speech recognition \cite{Han2020ContextNetIC}, and natural language processing \cite{Raffel2019ExploringTL, Clark2020ELECTRAPT}. While achieving remarkable advancements in performance, the architecture of DNN models has concurrently witnessed a significant increase in complexity and the computational parameters have experienced exponential growth \cite{Hestness2017DeepLS, Sattler2019UnderstandingTL}, creating a pressing challenge for deploying DNNs at the edge, in terms of memory, computation, and other relevant factors \cite{Sze2017EfficientPO, Sun2021DATE}. 

% Recently, the RISC-V vector processors\cite{Waterma2016EECS} are emerged as an appealing option for a diverse array of applications in both academic and industrial settings with the excellent capabilities of open-source development, efficient parallel processing, and scalability\cite{Razilov2022IWCMC, Johns2020FDL}.
% These processors, based on the exploration of data-level parallelism, can be specifically optimized for the efficient processing of vectorized data, allowing the same operation to be applied to multiple data elements simultaneously, which makes vector processors a good way to deal with the massive data computation tasks of DNN models\cite{Razilov2022IWCMC, Johns2020FDL}.
\rTwoCN{
RISC-V vector processors\cite{Waterma2016EECS} have recently emerged as an appealing option for a diverse array of applications in both academic and industrial settings, with excellent capabilities for open source development, efficient parallel processing, and scalability\cite{Razilov2022IWCMC, Johns2020FDL}. 
Based on the exploration of data-level parallelism, applying the same operation to multiple data elements simultaneously makes vector processors a good way to tackle computationally intensive tasks like DNNs\cite{Razilov2022IWCMC, Johns2020FDL}.}

% From an algorithmic point of view, 
\rTwoCN{However, the deployment of DNNs faces a pressing challenge in terms of memory, computation, and other relevant factors\cite{Sze2017EfficientPO, Sun2021DATE}.}
Quantizing DNN models is an effective way to handle large model sizes and large data computations with less impact on model accuracy\cite{hubara2016quantized, wang2019haq}.
\rTwoCN{Compared to full-precision DNN models, QNNs are more suitable for deployment on hardware.}
However, QNNs place new demands on vector processors capable of processing low-precision data. 
% Some previous research has concentrated on the implementation of vector architectures utilizing the RISC-V vector extension (RVV) standard instruction set, along with vector architectures aimed at enhancing computational throughput, such as Ara \cite{Cavalcante2020AraA1TVLSI, Cavalcante2022NewAra}. 
% However, these processors do not provide support for the prevalent low-precision data processing which utilized in modern DNNs. 
% Furthermore, they lack the flexibility required to perform DNN operations like convolution. Conversely, certain studies have acknowledged the necessity of low-precision data processing, but suffer from limitations in data throughput and computational efficiency\cite{Askarihemmat2023QuarkAI}.
% There are also processors available that can facilitate the deployment of low-precision DNN operators. However, their dataflow design exhibits suboptimal memory data utilization, expensive data handling, and significant computational overhead\cite{Theo2023sparq}.
% These processors face challenges in achieving a balance between supporting low-precision processing, facilitating flexible deployment of DNN operators, and achieving substantial computational throughput. Consequently, the deployment of DNNs remains a challenging task.
\rTwoCN{Some previous research such as Ara \cite{Cavalcante2020AraA1TVLSI, Cavalcante2022NewAra} do not provide support for the prevalent low-precision data processing which utilized in modern QNNs. Furthermore, they lack the flexibility required to perform DNN operations like convolution.
There are also processors available that can facilitate the deployment of low-precision operators\cite{Theo2023sparq, Askarihemmat2023QuarkAI}. But these processors face challenges in achieving a balance between facilitating flexible deployment of QNN operators and achieving substantial computational throughput.}
Consequently, the deployment of low-precision DNNs remains a challenging task.
To address the challenges above, we propose a configurable 
% multi-stage 
scalable multi-precision RISC-V vector processor, which integrates a systolic array unit to enable parametric multi-precision computation within extensible vector lanes. It possesses the capability to process quantized mixed low-precision DNN data concurrently, while also performing highly efficient long vector dot product computations and convolutional calculations with substantial data reuse.
Specifically, The contribution of this work can be summarized in the three following aspects:
% \noindent

\begin{enumerate}
    \item[\textbf{1)}]  \textbf{Customized instructions}: 
    % this paper proposes a customized instruction set \rTwoCN{with support for low-precision data} contains a configuration instruction, a vector load instruction, and a computation instruction. 
    \rTwoCN{this paper extends the RISC-V ISA with custom instructions used to support for low-precision data, meticulously crafted on exclusive extensions allocated within the framework of the standard RISC-V Vector extension (RVV) instruction set.}
    Supporting these new instructions, vector processors can achieve high effciency through parallelization of computations while maintaining the ﬂexibility of being programmable, and increase the performance of low-precision computations with the instructions.
    \item[\textbf{2)}] \textbf{Hardware architecture}: 
    % the deployment of a configurable multi-precision systolic array extends the parallelism dimension of processors, improving data reuse rate, facilitating low-precision data computations, and significantly increasing computational efficiency and hardware utilization.
    \rTwoCN{a scalable RISC-V vector processor is designed for efficient multi-precision DNN inference at high throughput. The scalable module, which integrates a systolic array unit, extends the dimension of parallel processing, increasing hardware utilization and computational efficiency.}
    % SPEED integrates a systolic array unit capable of handling multi-precision data within the scalable module lane to extend the dimension of parallel processing, thereby enhancing hardware utilisation and computational efficiency.}
    \item[\textbf{3)}] \textbf{Dataflow mapping}: \rTwoCN{ a hybrid dataflow mapping strategy is proposed which contains Feature map-First (FF) mapping strategy and Channel-First (CF) mapping strategy} for convolution computation. The method aim to achieve higher computational efficiency by flexibly adapting to different computations. 
    % Additionally, the bank conflict issue arising from meeting the high bandwidth requirements of pulsating arrays was resolved using a round-robin response method, leading to further reduction in the processor memory footprint of staging operands.

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The RISC-V vector processors are a type of processor architectures specifically optimized for the efficient processing of vectorized data, which exploit data-level parallelism, allowing the same operation to be applied to multiple data elements simultaneously. 
% This is primarily due to the advantages offered by their modular hardware architecture, vector lanes, which features flexible and customized extensible, that facilitate data parallelism.
% With the growing need for mixed-precision computing, vector processors offer compatibility across a range of data precisions, thereby facilitating the implementation of mixed-precision networks.
% Furthermore, The RISC-V vector processor presents the benefits of open-source development, efficient parallel processing, scalability, and mixed-precision capabilities. These features render it an appealing option for a diverse array of applications in both academic and industrial settings.\cite{Schmidhuber2014DeepLI}

%%%%%% 
%%Recently，the RISC-V vector processors are emerged as an appealing option for a diverse array of applications in both academic and industrial settings with the excellent capabilities of open-source development, efficient parallel processing, and scalability.
%%This processors are specifically optimized for the efficient processing of vectorized data, which exploit data-level parallelism, allowing the same operation to be applied to multiple data elements simultaneously.


% Deep neural network (DNN) \cite{Schmidhuber2014DeepLI} operations, such as matrix multiplications and convolutions, frequently necessitate the execution of the same operation on multiple data elements concurrently, making vectorized processing particularly well-suited for these tasks.
% Obviously, RISC-V vector processors is particularly valuable in deep learning and neural network applications, where a combination of high precision for accuracy and lower precision for computational efficiency is desired.
% As a result, RISC-V vector processors enable more efficient and scalable execution of DNNs than alternative architectures.

%With the remarkable successes of deep neural networks (DNNs) in the field of computer vision, the deployment of DNNs onto the embedded devices is attracting increasingly interests in both academia and industry.
%RISC-V vector processors, benifited from their excellent capabilities of open-source development, efficient parallel processing, and scalability, are emerged as an appealing hardware platform for acclerating the inference of DNNs.
%These processors, based on the exploration of data-level parallelism, can be specifically optimized for the efficient processing of vectorized data, allowing the same operation to be applied to multiple data elements simultaneously, which provides efficient support for the main operations in DNNs\cite{Schmidhuber2014DeepLI}.

%To pursue higher accuracy precision and computational efficiency, DNNs have adopted mixed-precision computing in the quantization processing of different layers, which puts forward high requirements for the vector processors.
% Several vector processors are currently under consideration, including Ara \cite{Cavalcante2019AraA1} and Sptaz \cite{Askarihemmat2023QuarkAI}, etc. 
% However, these processors exhibit low overall arithmetic capability due to the amount of data that each instruction can handle is limited to the number of extensible modules. 
% Furthermore, the extensible module suffers from poor data reuse capability, and the instructions become redundant when implementing conv-like operators. 
% Additionally, the processor supports an extensive range of data precision, which may not be suitable for some DNNs deployments.
% As a result, such processors are inadequate for supporting the mixed precision long dot-product operations that are prevalent in DNNs.

% To address the aforementioned challenges, a low-bit multi-precision vector processor, has been proposed. 
% This processor has the capability to process quantized mixed low-precision deep neural network (DNN) data in a parallel manner, whilst conducting efficient dot product operations. 
% By multiplexing the data, the number of instructions required for some operators, such as conv2d, has been significantly reduced. 
% To address the aforementioned challenges, we proposed a configurable multi-stage parallel multi-precision RISC-V vector processor. This processor integrates a systolic array unit to enable parametric multi-precision computation within extensible vector lanes. It possesses the capability to process quantized mixed low-precision deep neural network (DNN) data concurrently, while also performing highly efficient long vector dot product computations and convolutional calculations with substantial data reuse.
% Specifically, The contribution of this work can be summarized as the three following aspects:

% \begin{enumerate}
     % \item[1)] From the perspective of instruction set design: this paper proposes three categories of custom instructions: configuration instructions, loading instructions, and computation instructions. These instructions are tailored for various DNN layer computations and exhibit significant flexibility. Briefly, They are specifically designed for DNN processing.
     % \item[2)] From the perspective of hardware architecture: the deployment of a configurable multi-precision systolic array has overcome the precision limitations of the original vector processor. Additionally, this enhancement has resulted in improved data parallelism and data utilization, enabling an increase in the amount of data processed per instruction and enhancing computational efficiency.
     % \item[3)] From the perspective of dataflow design: three data flow allocation methods were devised: matrix computation mode, HWC mode for convolution computation, and CHW mode for convolution computation. These methods aim to achieve higher computational efficiency by adapting to different types of computations. Additionally, the bank conflict issue arising from meeting the high bandwidth requirements of pulsating arrays was resolved using a polling response method, leading to further reduction in computation cycles per instruction.
% \end{enumerate}

% Consequently, proposed hardware has the potential to be a highly effective edge-side processor, enabling the deployment of DNNs with large amounts of data and high computational demands.


% A citation Example: \cite{mallasen2022percival}

==> 2-bkg-r1.tex <==
\section{Background}\label{sec:bkg}
% \vspace{1em}
% A. Deep Neural Network search
\subsection{Analysis of DNN Operators}
In the AI application field, convolutional neural network (CNN) based and Transformer-based DNNs are widely used for their broad applicability in different domains.
These two architectures differ in design and algorithm, which leads to their respective advantages and characteristics in different tasks. 
We analyze the basic operators of these two DNNs in the following section.

CNN models typically consist of convolution, pooling, and fully-connected layers, with convolution computation playing a crucial role in the inference of CNN models.
Standard convolution (CONV) and point-wise convolution (PWCV) exhibit high computational complexity relative to storage requirements, benefiting from the extensive reuse of input feature map and weight kernels.
In depth-wise convolution (DWCV), the results are not perform accumulated in the input channel dimension, resulting in a more balanced computational complexity and storage bandwidth.
In addition, convolution computation can be reorganized using the im2col function to transform data into matrix form, and then computed using the General Matrix Multiply (GeMM) method~\cite{Jacob2018GEMM}.
Most NLP and Vision Transformer models are based on the transformer architecture. 
The transformer architecture consists of attention, fully-connected, and nonlinear layers. 
Attention layers are a important component of the transformer architecture, which uses the input matrices to compute the attention matrix.
The computation involves  a large number of matrix multiplication operations, resulting in a high ratio of computation to storage requirements.
\subsection{Motivation for Vector Processor with Tensor Unit}
The inference of a complete DNN consists of two types of computations: vector computations for pooling layer and non-linear layer computations, and tensor computations. 
Tensor computations include convolution and matrix multiplication computations, both of which consist of multiply-and-accumulate (MAC) operations.
Tensor computations dominate the inference of DNN models. 
However, vector processors typically decompose tensors into vectors for acceleration, leading to reduce computation efficiency.
Earlier NPU architectures are designed only with a homogeneous processor to accelerate only tensor computations, or support a limited set of operators, which prevented them from achieving complete DNN models inference~\cite{Jouppi2021TPU}.
Therefore, it is necessary to design a vector processor that can efficiently support tensor computation while maximizing the utilization of storage resources.
Introducing a tensor unit within the scalable module of the vector processor emerges as a promising solution. 
First, the tensor unit and vector processing unit share storage resources, which improves the utilization of on-chip memory and the opportunity for data reuse. 
Second, this expansion further extends the dimension of parallelism for tensor computations that can be configured.
Based on the above considerations, this work incorporates a parameterized tensor unit to the scalable module of a vector processor to achieve efficient inference for DNNs.
% DNNs have exhibited notable achievements across a multitude of domains, including computer vision \cite{Ren2015FasterRT, Bochkovskiy2020YOLOv4OS}, speech recognition \cite{Chan2016ListenAA, Han2020ContextNetIC}, and natural language processing \cite{Raffel2019ExploringTL, Clark2020ELECTRAPT}. 
% In prior research, DNNs have been optimized to achieve data compression with precision ranging from 1 to 8 bits per layer, while maintaining acceptable levels of accuracy loss. Among the commonly used types, 4-bit and 8-bit precision have been widely employed\cite{Zhou2016DoReFaNetTL, Li2022APE, Yin2019AnER}.
% Table~\ref{tab:analyzation} presents a comprehensive overview of frequently employed mixed-precision networks. 

% As can be seen from the table, the loss of accuracy is small or even negligible when performing network quantization with multi-precisions.
% For the practical implementation of DNNs. The processor is specifically designed to support multiple low-precision computations, enabling efficient processing of quantized mixed low-precision DNN models.
% Nevertheless, it has been observed that as neural networks grow deeper in terms of layer depth, the accuracy of these networks declines significantly when data precision is reduced to less than 8 bits.\cite{Rajagopal2018AccurateAE, Jain2018CompensatedDNNEE}
% Conversely, a higher data precision of 16 bits is found to better safeguard the accuracy of the network.\cite{Rajagopal2018AccurateAE}


% In order to cater to the requirements of larger models operating under varying data precision scenarios, accelerators need to exhibit flexibility in terms of configurable precision and compatibility with lower precision functionalities.  
% Therefore, the vector processor proposed in this paper is capable of handling data processing in mixed precision of 16bit/ 8bit/ 4bit.

% B. Vector processors
% \subsection{Vector processors}
% % \rOneFC{
% % RISC-V, an open-source instruction set architecture (ISA) \cite{Waterma2016EECS}, offers modularity and extensibility for processor design. While RISC-V scalar processors handle individual instructions on scalar data, recent studies explore integrating RISC-V with vector architectures to boost throughput.}
% \rOneFC{Ara\cite{Cavalcante2022NewAra} uses scalable lanes for parallel computations, but it's limited to byte computation and underperforms for sub-byte tasks. Quark\cite{Askarihemmat2023QuarkAI} and Sparq\cite{Theo2023sparq} accelerate ultra-low-precision data vectors but struggle with 16-bit data.}
% \rOneFC{In contrast, SPEED extends RISC-V with customized instructions to accelerate low-precision vector computation and incorporates multi-modal computational dataflows for DNN operators. It employs a configurable multi-dimensional parallel lanes using a systolic array, effectively addressing challenges faced by previous processors. This makes SPEED a distinctive and promising vector processor for diverse applications.}


==> 2-bkg.tex <==
\section{Background}\label{sec:bkg}
% \vspace{1em}
% A. Deep Neural Network search
\subsection{Multiple-Precision Deep Neural Networks}

DNNs \cite{Schmidhuber2014DeepLI, Hanif2022CoNLoCNNEC, Chakraborty2019ConstructingEM} have exhibited notable achievements across a multitude of domains, including computer vision \cite{Ren2015FasterRT, Bochkovskiy2020YOLOv4OS}, speech recognition \cite{Chan2016ListenAA, Han2020ContextNetIC}, and natural language processing \cite{Raffel2019ExploringTL, Clark2020ELECTRAPT}. 
In prior research, DNNs have been optimized to achieve data compression with precision ranging from 1 to 8 bits per layer, while maintaining acceptable levels of accuracy loss. Among the commonly used types, 4-bit and 8-bit precision have been widely employed\cite{Zhou2016DoReFaNetTL, Li2022APE, Yin2019AnER}.
Table~\ref{tab:analyzation} presents a comprehensive overview of frequently employed mixed-precision networks. 

As can be seen from the table, the loss of accuracy is small or even negligible when performing network quantization with multi-precisions.
For the practical implementation of DNNs. The processor is specifically designed to support multiple low-precision computations, enabling efficient processing of quantized mixed low-precision DNN models.
% Nevertheless, it has been observed that as neural networks grow deeper in terms of layer depth, the accuracy of these networks declines significantly when data precision is reduced to less than 8 bits.\cite{Rajagopal2018AccurateAE, Jain2018CompensatedDNNEE}
% Conversely, a higher data precision of 16 bits is found to better safeguard the accuracy of the network.\cite{Rajagopal2018AccurateAE}

\begin{table}[!hb]
\centering
% \tabcolsep= 0.015\linewidth
\resizebox{0.48\textwidth}{!}{
\begin{threeparttable}
\caption{Accuracy Analyzation of the mix-precision networks}
\label{tab:analyzation}
\begin{tabular}{ccccc}
% \tabcolsep= 0.015\linewidth
% {\linewidth}{@{}LLLL@{}} 
\toprule
 Model   &  Dataset     &  \begin{tabular}[c]{@{}c@{}}Data\\ Precision\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}FP32\\ Accuracy\end{tabular} &  Accuracy   \\ 
\midrule
 Resnet18 \cite{Lin2022LGLSQLG} &ImageNet &  4 &  69.76\% &  70.78\%  \\ 
\multirow{2}{*}{ MF-DFP \cite{Tann2017DAC}}  
 &  CIFAR-10 &  4/8  & 81.53\% & 80.77\%   \\
 &  ImageNet &  4/8  &  79.88\% &  79.13\% \\

VGG16 \cite{Rajagopal2018AccurateAE} & ImageNet & 16 &  86.64\% &  86.65\%   \\
ResNet-50 \cite{Rajagopal2018AccurateAE} &  ImageNet & 16 &  89.91\% &  89.90\%   \\
\bottomrule
\end{tabular}

\end{threeparttable}
}
\vspace{-0.4cm}
\end{table}

% In order to cater to the requirements of larger models operating under varying data precision scenarios, accelerators need to exhibit flexibility in terms of configurable precision and compatibility with lower precision functionalities.  
% Therefore, the vector processor proposed in this paper is capable of handling data processing in mixed precision of 16bit/ 8bit/ 4bit.

% B. Vector processors
\subsection{Vector processors}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  wangshifu's new draft  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
RISC-V is an open-source instruction set architecture (ISA) \cite{Waterma2016EECS} that provides a modular and extensible framework for designing processors. The RISC-V scalar processors are a subset of RISC-V processors that handle individual instructions on scalar data. 
Due to the inherent benefits of the RISC-V scalar processor's open-source nature, along with its notable modularity and extensibility, it enables anyone to personalize the design to meet specific requirements. Consequently, this adaptability expands the range of potential application scenarios for scalar processors, encompassing both embedded devices \cite{zaruba2019CVA6} and high-performance computing environments \cite{Benini2017RIC5Y}.

Nevertheless, RISC-V scalar processors are limited to processing scalar data (one elements). To increase throughput of processor, recent studies have explored the integration of RISC-V nature with vector architectures, aiming to develop more efficient RISC-V processor designs.

% Ara\cite{Cavalcante2019AraA1}, a vector processor based on the standard RISC-V instruction set, enhancing computational efficiency by utilizing configurable scalable lanes to execute parallel computations with a 64-bit bit-width. However, Ara's support is limited to byte computation and this limitation makes the architecture sub-optimal for sub-byte computing. Furthermore, during matrix and convolution computations commonly employed in DNNs, Ara employs a dataflow scheme that leverages vector-scalar computation for each instruction, aiming to enhance data utilization. However, this approach leads to reduced throughput and underutilization of the vector architecture's parallel capabilities.

% Quark\cite{Askarihemmat2023QuarkAI} and Sparq\cite{Theo2023sparq}, have the capability to facilitate sub-byte vector computation by employing customised instructions. However, their effectiveness is limited to accelerating computations involving ultra-low-precision data vectors. Regrettably, the performance of 16-bit data computation remains inadequate. Furthermore, a satisfactory solution to the challenge of balancing data utilization and throughput through an efficient dataflow design method is currently lacking.

% Compared to existing research, SPEED is a distinctive vector processor that extends the RISC-V ISA by adding customised instructions to accelerate sub-byte vector computation, incorporates multi-modal computational dataflows for deploying DNN operators and incorporates a configurable multi-dimensional parallel lanes by adding systolic array. These advancements effectively addresses the enduring challenges faced by preceding processors.













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State-of-The-Art RISC-V vector processor have demonstrated capability in supporting mixed-precision computation; however, their supported data precision is limited, with a minimum precision of 8 bits. Furthermore, in the context of matrix processing and convolution calculations, the amount of data that can be processed in a single instruction is constrained by the number of expandable modules, as depicted in Figure 1. Specifically, N expandable modules are available, and a single instruction can load N data elements simultaneously, which are then multiplied with a single data element. The multiplication of (1xN) by (Nx1) matrices necessitates 1 load instruction and N compute instructions. Such computational capability is insufficient to meet the requirements of deploying a large number of data processing operators.

% Ara is a lane-based open-source RISC-V vector processor that currently supports RISC-V V extension v1.0.  It is highly configurable and offers greater generality, with potential for deployment in multi-core networks. Several other vector processors have limitations such as small maximum bit width of vector registers and a limited number of computational units, or they support lower versions of extensions. Hence, these vector processors are not considered in this paper.

% Systolic array is a classical computational module that support data reuse and parallel processing of multiple matrix multiplication and convolution operations. In this work, we propose to integrate a multi-processing mode and mixed-precision Systolic array unit into Ara's Lane, leveraging the strengths of both approaches and addressing the limitations of the aforementioned processors.

==> 3-design.tex <==
% Para. 1 - 概述
% 核心目的：介绍SPEED架构及其在多精度深度神经网络（DNN）推理中的应用。
% 1. 简述SPEED架构，它是一个基于RVV v1.0 ISA的可扩展RVV处理器，专为高吞吐量多精度DNN推理而设计。
% 2. 强调SPEED与RISC-V标量核心和外部内存的紧密耦合，以及其在定制指令和微架构方面的创新。

% Para. 2 - 定制指令的动机与设计
% 核心目的：阐述为何需要为DNN构建定制指令，并详细介绍这些指令。
% 1. 分析现有RISC-V官方向量扩展指令集的不足，指出其在处理DNN推理时的复杂性和资源消耗问题。
% 2. 描述定制指令的设计原则，包括VSACFG、VSALD、VSAM和VSAC等指令的详细功能和实现方式。

% 过渡段落 - 定制指令与微架构的衔接
% 核心目的：简洁地过渡到微架构的介绍，强调定制指令与硬件设计的紧密联系。
% 1. 指出定制指令的设计如何直接影响微架构的实现，为微架构的高效执行提供基础。
% 2. 预告微架构部分将展示硬件组件如何支持这些指令，以及它们如何共同作用于提升DNN推理性能。

% Para. 3 - SPEED的微架构
% 核心目的：详细介绍SPEED的微架构设计，展示如何支持定制指令的执行。
% 1. 描述SPEED微架构的硬件组成，包括向量指令解码单元（VIDU）、向量加载单元（VLDU）和可扩展模块（lane）。
% 2. 详细说明多精度张量单元（MPTU）的层次结构，以及其如何实现高效的多精度数据并行处理和数据重用。

\section{The Proposed SPEED Architecture}\label{sec: Archi_design}
% SPEED is a scalable RVV processor augmented with customized instructions enabling high-throughput multi-precision DNN inference, which is built on the RVV v1.0 ISA. Additionally, the RVV processor is tightly coupled to a RISC-V scalar core for programmable instructions and an external memory for fetching necessary data. In this section, SPEED will be described from two perspectives: customized instructions, micro-architecture.
\jOneFC{SPEED is a scalable RVV processor enabling area-efficient and high-throughput MP-DNN inference, built upon the RVV v1.0 ISA. 
It is tightly coupled to a RISC-V scalar core for flexible programming and equipped with an external memory for efficient data retrieval. 
% SPEED meets the varying needs of MP-DNN inference by effectively combining easy-to-use efficient dedicated instructions with the power needed for precise calculations at different levels of detail
% SPEED caters to the evolving challenges of MP-DNN inference by fusing a flexible set of instructions customized for precision-scalable DNN operations with a hardware architecture that efficiently enables MP-DNN operations.
% This section will outline SPEED's architecture, focusing on its customized instructions and innovative micro-architecture that together enhance DNN inference efficiency.
SPEED is designed to address the evolving challenges of MP-DNN inference by integrating specialized instructions with an efficient hardware architecture, and this section will detail how these two innovations enhance MP-DNN inference efficiency.
}
\begin{figure}[!htbp]
  \centering
    \includegraphics[width=0.92\columnwidth]{figures/customized_instr.pdf}
      % \caption{An analysis of NNs acceleration from the operator to ISA levels.}
      \caption{\jOneFC{Customized vector instructions of SPEED drive enhanced computational efficiency in operators for MP-DNN inference.}}
        \label{fig:customized_instr}
\end{figure} 
% In recent years, the neural networks widely used in the field of AI are mainly divided into three categories: convolutional neural network (CNN)-based~\cite{Liu2015VGG16, Szegedy2015Googlenet, Sandler2018MobileNet}, transformer-based ~\cite{dosovitskiy2021an, Yang2019XLNet, Rao2021DynamicViT}, and hybrid structures that combine CNNs and transformers~\cite{Liu2022SwinTransformer, Ng2022Convmixer, Yuan2021ViT}. 

% \subsection{Mapping DNN Operators onto Hardware via Instructions}\label{subsec: mapping}
% \subsection{Motivations to Building Customized Instructions for DNNs}\label{subsec: motivations}
\subsection{Motivations for Customized Vector Instructions}\label{subsec: motivations}
% These network models have demonstrated excellent performance in different domains, and their differences are determined by their network structures and basic operators.
% CNN models are mainly based on convolutional operations, which include standard convolution (CONV), point-wise convolution (PWCV), and depth-wise convolution (DWCV)~\cite{Liu2015VGG16, He2016ResNet, Sandler2018MobileNet}.
% CONV and PWCV exhibit high high computational complexity relative to storage requirements, benefiting from the extensive reuse of input feature maps and weight kernels.
% However, in the DWCV, the results are not perform accumulated in the input channel dimension, resulting in relatively consistent computation and storage requirements.
% Attention layers are a important component of the transformer architecture, which consist of matrix multiplication operations and exhibits a relatively high computational and storage requirement ratio.

% To efficiently implement DNN inference on vector processors, a sequence of vector instructions is typically employed to describe the computation process of operators.
% Though RISC-V provides an official vector extension instruction set, it is designed for general-purpose computing and is too complex for specialized DNN operators. 
% And the official data arrangement method between scalable modules is relatively simple.
% \rOneCN{Though RISC-V provides an official vector extension instruction set, it is designed for general-purpose computing without consideration of specific operators. 
% And the data arrangement method under official RVV load instructions is ordered allocation with no data reuse across the scalable modules.
% Therefore, the deployment of official ISA requires complex groups of extensive fine-grained instructions when processing operators with different computing-storage requirements in DNN inference.
% % Additionally, the process of instruction fetching and decoding increases the hardware resource consumption of the processor front-end, resulting in certain limitations on the computational efficiency of the computing unit.
% The abundance of instructions complicate the decode unit, leading to increased hardware overhead and power consumption. 
% Moreover, the prolonged process of instruction decoding resulting in certain limitations on the computing efficiency of the computing module.}
% Based on the above analysis, there is a certain optimization space in the instruction set design.
% % Through customized arithmetic instructions for DNN operators and the addition of data arrangement instructions, specific operators with various computation-storage requirements in DNNs can be processed more efficiently, thus achieving efficient DNN inference.
% \rOneCN{To reduce the number of instructions in DNN inference, multiple customized instructions are designed.
% These instructions include parameter configuration for specific operators, enhancing data reuse opportunities between scalable modules, and specific operator computation.}
% Detailed description and the implement of customized vector instructions are provided below.
% \rTwoCN{\textbf{New version of Motivations begins}}


% The RISC-V architecture has garnered widespread acclaim due to its open-source nature and extensibility. 
% However, the official RVV v1.0 ISA extension, while powerful for general-purpose computing, may encounters limitations when executing MP-DNN inference.
% The RVV ISA extension~\cite{RVVExtension}, which is powerful for general-purpose computing, encounters some limitations when being leveraged to perform MP-DNN inference~\cite{Zhao2023HIPU}.
\jOneFC{While the RVV ISA extension~\cite{RVVExtension} is powerful for general-purpose computing, it encounters some limitations when being leveraged to perform MP-DNN inference~\cite{Zhao2023HIPU}.}
As shown in Fig.~\ref{fig:customized_instr}, MP-DNNs can be decomposed into various operators.
% \rThreeCN{with convolution operators accounting for more than 95\% of the total inference time~\cite{PCONV2020AAAI}.
\jOneFC{Note that convolution operators in the popular convolutional neural networks (CNNs) account for more than 95\% of the total inference time~\cite{PCONV2020AAAI}, which include standard convolution (CONV), point-wise convolution (PWCV), and depth-wise convolution (DWCV)~\cite{Liu2015VGG16, He2016ResNet, Sandler2018MobileNet}, constituting the majority of the computational workload in CNNs.}
% constitute the majority of the computational workload.}
% \rThreeCN{These computationally intensive convolution operators, including standard convolution (CONV), point-wise convolution (PWCV), and depth-wise convolution (DWCV)~\cite{Liu2015VGG16, He2016ResNet, Sandler2018MobileNet},
% constitute the majority of the computational workload.}
% As shown in Fig.~\ref{fig:customized_instr}, MP-DNNs can be decomposed into various operators, among which the computationally intensive convolutional operators, including standard convolution (CONV), point-wise convolution (PWCV), and depth-wise convolution (DWCV)~\cite{Liu2015VGG16, He2016ResNet, Sandler2018MobileNet}, 
% constituting the majority of computational workload. 
% Additionally, the matrix multiplication (MM) operations within the encoder module of Transformer models~\cite{fang2022algorithm} also account for a significant proportion of computational demand.
% \rThreeCN{Moreover, in Transformer models~\cite{dosovitskiy2021an, Yang2019XLNet, Rao2021DynamicViT, fang2022algorithm}, another popular DNN architecture, matrix multiplication (MM) operations also exhibit a high computational demand.
% These operations account for 95\% of the consumed parameters and 65$\sim$85\% of all computations~\cite{GPT32022NeurIPS}.}
\jOneFC{Similarly, matrix multiplication (MM) operations in Transformer models~\cite{dosovitskiy2021an, Yang2019XLNet, Rao2021DynamicViT, fang2022algorithm} are computationally expensive, accounting for a significant portion of the model's parameters and computations~\cite{GPT32022NeurIPS}.}
% \rThreeCN{The distinctive computational characteristics of these operators are not optimally addressed by processors based on official RVV instructions, such as Ara, presenting significant challenges for the efficient deployment of MP-DNN inference~\cite{Zhao2023HIPU}.}
\jOneFC{However, processors relying solely on the official RVV instruction set, such as Ara~\cite{Cavalcante2022NewAra}, struggle to efficiently handle the unique computational characteristics of these operators~\cite{Zhao2023HIPU}.}
% The unique computing characteristics of these operators are not optimally addressed by the RVV instructions, presenting significant challenges for efficient MP-DNN inference~\cite{Zhao2023HIPU}.
% These challenges encompass the limited range of supported inference precisions, the extensive number of instructions required for inference, and the deficiency in leveraging the reuse opportunities of scalable modules. 
% These issues not only lead to decoding delays that impair overall computational efficiency but also increase hardware resource consumption due to the complexity of the decoding units.
\jOneFC{The arising challenges include limited supported precisions, a high instruction count, and the inefficiency in leveraging the reuse opportunities of scalable modules, which not only lead to decoding delays that impair overall computational efficiency but also increase hardware resource consumption due to the complexity of the decoding units.}
% These limitations lead to decoding delays, reduced overall efficiency, and increased hardware resource consumption due to complex decoding units.}

% \rTwoCN{
% To address these issues, we propose a series of targeted optimization measures. 
% As shown in Fig.~\ref{fig:customized_instr}, firstly, in terms of parameter configuration, we can support a broader range of precisions through parameter adjustments and simplify the decoding process for other instructions. 
% Secondly, regarding data arrangement strategies, we can enhance computational efficiency by implementing data reuse at the level of scalable modules. 
% Lastly, in the realm of arithmetic processing, we propose specialized instructions to directly execute matrix-matrix or matrix-vector operations, thereby reducing the reliance on general arithmetic instructions.}
% \rThreeCN{To address the limitations above, SPEED introduces a series of targeted optimization measures as shown in Fig.~\ref{fig:customized_instr}.
% The proposed optimization measures aim to simplify the configuration of operator parameters, enhance data reuse across scalable modules, and directly compute specific operator functions, thereby improving the overall efficiency of MP-DNN inference.}
To address the limitations above, SPEED introduces several optimization techniques when designing customized RVV instructions as illustrated in Fig.~\ref{fig:customized_instr}. \jOneFC{These optimizations aim to simplify operator parameter configuration, enhance data reuse across scalable modules, and directly compute specific operator functions, thereby improving the overall efficiency of MP-DNN inference.}

% \rTwoCN{
% Based on these optimization strategies, we further propose a suite of custom instructions tailored to specific MP-DNN operators, aim to simplify the configuration of operator parameters, enhance data reuse across scalable modules, and directly compute specific operator functions, thereby improving the overall efficiency of MP-DNN inference while minimizing the hardware overheads.}

% \rTwoCN{\textbf{New version ends}}

% \jOneFC{The official RVV v1.0 ISA extension, while powerful for general-purpose computing, encounters limitations when being leveraged to perform MP-DNN inference.
% As shown in Fig.~\ref{fig:customized_instr}, MP-DNNs can be decomposed into various operators, among which the compute-intensive convolutional operators, including standard convolutions (CONV), point-wise convolutions (PWCV), and depth-wise convolutions (DWCV) \cite{Liu2015VGG16, He2016ResNet, Sandler2018MobileNet}, constitute the majority of the computational workload.
% The unique computational demands of these operators are not optimally addressed by the RVV instructions, presenting significant challenges for efficient MP-DNN inference.
% For instance, standard CONV operations with varying kernel sizes and strides necessitate complex sequences of instructions to manage the spatial and channel-wise data transformations. 
% PWCV operations, though simpler, still require efficient handling of the one-by-one kernel multiplications across all channels. 
% DWCV operations, which process each input channel independently, can benefit from instructions that optimize the computation and storage for these operations.
% Furthermore, the attention layers in Transformer models\cite{fang2022algorithm}, which involve extensive matrix multiplications (MMs), are not optimally supported by the official RVV extension, leading to suboptimal resource utilization and increased computational overhead.
% To address the limitations above, SPEED introduces a suite of custom vector instructions tailored for MP-DNN operations.
% The proposed customized vector instructions aim to simplify the configuration of operator parameters, enhance data reuse across scalable modules, and directly compute specific operator functions, thereby improving the overall efficiency of MP-DNN inference.
% }

\subsection{Customized Efficient Vector Instructions of SPEED}\label{subsec: instr_design}

% \textbf{Design of Customized Vector Instructions.}
% To facilitate efficient inference of multi-precision DNNs, various DNN models are decomposed into a set of specific operators for decreasing complexity, as shown in Fig.~\ref{fig:customized_instr}. 
\rTwoCN{Based on the analysis of operator deployment for efficient MP-DNN inference, as shown in Fig.~\ref{fig:customized_instr}, several customized instructions are proposed using the reserved user-defined encoding space in RISC-V.}
\rThreeCN{Specifically, the customized instructions mainly contain the configuration-setting (\texttt{VSACFG}), memory access (\texttt{VSALD}), and arithmetic (\texttt{VSAM}, \texttt{VSAC}).}
% The detailed descriptions of each instruction are as follows.}

\texttt{VSACFG} serves as an efficient vector configuration-setting instruction that effectively provides the necessary information of specific operators, such as data precision (4-, 8-, and 16-bit), size of convolution kernel (1, 3, 5, and 7), and dataflow mapping strategy.
The above information are decoded according to the value of $zimm$[8:0] and $uimm$[4:0], respectively, and then specified in a control register ($rd$) for the subsequent computations, as shown in Fig.~\ref{fig:customized_instr}.

\texttt{VSALD} is a customized vector memory access instruction designed to efficiently load data from the external memory. 
% \rThreeCN{Compared to the sequential allocation operation of the official RVV load instruction \texttt{VLE}, 
% the data arrangement of \texttt{VSALD} enables the data loaded from external memory and multi-broadcasted to each scalable modules, thereby improving data reuse opportunities.}
\jOneFC{Unlike the official RVV load instruction \texttt{VLE} that performs sequential allocation, \texttt{VSALD} facilitates data reuse by enabling simultaneous loading and multi-broadcasting of data from external memory to individual scalable modules.}
% the loaded data from the external memory are broadcast to each lane for improving data reuse.  
The vector load instruction \texttt{VSALD} is as follows:
% \begin{equation}
$$ \texttt{VSALD(width).v\quad vd, (rs)}\text{,} $$
% \end{equation}
where the vector load moves data from external memory with address (\texttt{rs}) to the vector register \texttt{vd} at the precision which is determined by \texttt{width}. 

\texttt{VSAM} and \texttt{VSAC} are customized arithmetic instructions that exploit data parallelism for matrix-matrix operations and matrix-vector operations, respectively.
% , thereby enhancing computational efficiency.
% The RVV official instructions are limited to processing vectors of the same length. 
% Consequently, matrix-matrix/vector operations are decomposed into multiple vectors and then processed through a sequence of vector-vector or vector-scalar operations. 
% This approach introduces performance overheads, including the additional data access and arithmetic instructions, coupled with increased usage of vector registers.
% \rThreeCN{Prior works~\cite{Cavalcante2022NewAra, Cavalcante2020AraA1TVLSI, Askarihemmat2023QuarkAI, Theo2023sparq, Perotti2023Yun} are limited by fixed parallelism dimension, generally decomposing matrix-matrix/vector operations into multiple vector-vector or vector-scalar operations.}
% This method requires more computation steps, increases the number of data movement and arithmetic instructions, and requires more vector registers to store data, thus increasing resource consumption.
\jOneFC{Unlike the arithmetic instructions in prior works~\cite{Cavalcante2022NewAra, Cavalcante2020AraA1TVLSI, Askarihemmat2023QuarkAI, Theo2023sparq, Perotti2023Yun} that are limited by a single parallelism dimension, the proposed \texttt{VSAM} and \texttt{VSAC} can directly perform operations on entire matrices or vectors within multiple parallelism dimensions.}
\jOneFC{This eliminates the need to decompose operations into multiple smaller ones, significantly reducing the number of instructions, data movements, and required vector registers.}
% \rThreeCN{In contrast, \texttt{VSAM} and \texttt{VSAC} instructions directly perform operations on matrix-matrix/vector, reducing the number of instructions and the consumption of storage space when processing the same tasks.}
\jOneFC{Hence, \texttt{VSAM} and \texttt{VSAC} offer improved computational efficiency and lower resource consumption.}
% The vector arithmetic instruction \texttt{VSAM} and \texttt{VSAC} are structured as follows:
The \texttt{VSAM} and \texttt{VSAC}  vector arithmetic instructions are as follows:
$$ \begin{cases}\texttt{VSAM.vv\quad vd,\,vs1,\,vs2}\text{,} \\ \texttt{VSAC.vv\quad vd,\,vs1,\,vs2}\text{,}\end{cases}$$
% 对齐符放在想要对齐的地方就可以了
% $$\begin{cases}\{vlb,vlh,vlw\}~VR_d,&(R_{s1})imm&\\\{vsb,vsh,vsw\}~R_{s2},&(R_{s1})imm&\end{cases}$$
% where \texttt{vs1} and \texttt{vs2} are the source vector registers holding the input matrices/vectors for matrix operations. 
% \jOneFC{where \texttt{vs1} and \texttt{vs2} are source vector registers holding the input operands, and \texttt{vd} is the destination register that stores the result.}
\jOneFC{where \texttt{vs1} and \texttt{vs2} are source vector registers holding the input operands. The computation result is stored in the destination vector register, denoted as \texttt{vd}, enabling efficient post-processing with vector instructions on chip and eliminating the need for additional off-chip communication.}

% The computation result is stored in the destination vector register (vd), enabling efficient post-processing with vector instructions (e.g., data analysis or accumulation)  within the chip, eliminating the need for additional off-chip communication.}
% The matrix computation result is stored in the vector register (\texttt{vd}), 
% \rThreeCN{which allows efficient post-processing using vector instructions, such as data analysis or accumulation, eliminating the requirement for additional off-chip communication.}
% \jOneFC{This in-register processing allows for efficient post-processing using other vector instructions, such as data analysis or accumulation, without requiring additional off-chip communication for intermediate results.}
\begin{figure}[!htbp]
  \centering
    \includegraphics[width=1\columnwidth]{figures/instr_compare.pdf}
      % \caption{The timeline comparison between SPEED and Ara when performing an INT16 MM operator. The example depicts the instruction flows and register file usage of SPEED’s and Ara’s scalable module, respectively.}
      \caption{\jOneFC{Comparison of SPEED and Ara when performing an INT16 MM operator. SPEED leverages fewer instructions, requires smaller number of register files, and achieves fewer computing cycles over Ara.}}
        \label{fig:instr_compare}
\end{figure}

% \textbf{Implement of Customized Vector Instructions.}
% \rOneCN{\textbf{Example of Customized Vector Instructions Sequence}}
% To showcase the advantages of customized vector instructions, we present the sequential instructions of SPEED and Ara, respectively, when processing a 4$\times$8 MM operator at 16-bit, and provide the corresponding processing cycles and register usage.
\jOneFC{To demonstrate the advantages of customized vector instructions, we compare the processing instruction sequences of SPEED and Ara for a 4$\times$8 MM operator at 16-bit precision with a focus on the processing cycles and register usage for both architectures.}
% As depicted in Fig.~\ref{fig:instr_compare}, both SPEED and Ara require setup and compute stages for parameter configuration and subsequent computation, respectively. 
% , making it more computationally efficient than Ara.
\jOneFC{As shown in Fig.~\ref{fig:instr_compare}, both SPEED and Ara involve setup and compute stages for parameter configuration and execution, respectively. 
The setup stage configures parameters for the subsequent computation.}
\rOneCN{Specifically, in the setup stage, both processors utilize the \texttt{VSETVLI} instruction to set the application vector length, managing computational resources for vector operations. SPEED, however, introduces the \texttt{VSACFG} instruction, enabling direct configuration of parameters crucial for matrix and convolution computations.}
% In the compute stage, SPEED employs the \texttt{VSALD} instruction to realize data multi-broadcast between the scalable modules for efficient data reuse. 
\jOneFC{Moving to the compute stage, SPEED leverages the \texttt{VSALD} instruction to achieve multi-broadcasting of data across scalable modules, facilitating efficient data reuse.}
% In contrast, Fig.~\ref{fig:instr_compare} shows that Ara relies on 16 individual VMACC instructions, demonstrating the redundancy addressed by SPEED's custom vector instructions.}
% \rThreeCN{In addition, as shown in Fig.~\ref{fig:instr_compare}, Ara relies on 16 arithmetic instructions, namely \texttt{VMACC}, while SPEED only needs four \texttt{VSAM} instructions during the compute stage.}
\jOneFC{In addition, as shown in Fig.~\ref{fig:instr_compare}, Ara relies on 16 individual arithmetic instructions, namely \texttt{VMACC}, for computations, whereas SPEED achieves the same result with only four \texttt{VSAM} instructions.}
\rThreeCN{Finally, both Ara and SPEED employ four \texttt{VSE} instructions to store the computation results.}
\jOneFC{By employing customized vector instructions tailored to specific operators, SPEED achieves a significant efficiency improvement compared to Ara. 
In this case, SPEED utilizes 46\% fewer instructions and 50\% fewer registers, leading to a 1.4$\times$ throughput boost over Ara.}
% \jOneFC{By leveraging customized vector instructions for specific operators, 
% Our processor uses 46\% fewer instructions and 50\% fewer registers than Ara.
% The significant reduction in instruction count and cycles contributes to a 1.4$\times$ improvement in throughput for SPEED.
% SPEED uses 46\% fewer instructions and 50\% fewer registers than Ara in this case, leading to a 1.4$\times$ throughput improvement over Ara.}
% Furthermore, Ara requires multiple data access instructions for vector load and store, while SPEED manages with just three load instructions and two store instructions. 

\begin{figure}[!htbp]
  \centering
    \includegraphics[width=1\columnwidth]{figures/archi.pdf}
      \caption{Micro-architecture of SPEED, the proposed RVV processor.}
        \label{fig:micro_arichi}
\end{figure}

\subsection{Micro-architecture of SPEED}
% \rOneCN{Waiting for modified!!!}
% DNN inference typically involves two types of computation: vector computations and tensor computations. Vector computations include normalization, pooling and non-linear activation operations, while tensor computations mainly consist of convolution and matrix multiplication operations composed of multiply-accumulate (MAC) operations.
% However, NPU architectures typically adopt homogeneous designs, focusing on accelerating tensor computations or supporting only a limited set of vector operators~\cite{Jouppi2021TPU}. 
% This limitation results in their inability to fully implement inference for the entire DNNs.
% Additionally, vector processors lack specialized optimizations for tensor computations and typically decompose tensors into vectors for processing, which leads to relatively inefficient DNN inference.
% Therefore, it is important to design a vector processor capable of effectively handling both vector and tensor computations.
% \rOneCN{
% To achieve efficient inference of quantized DNNs, a vector processor integrating a parameterized multi-precision tensor unit (MPTU) within the scalable module is proposed. 
% The incorporation method provides a more flexible choice of data parallelism configuration, enabling maximum matching of throughput requirements for different applications.
% At the same time, by sharing the storage of MPTU with the original vector units, the existing on-chip resources can be fully utilized, avoiding additional storage cost and data movement.}
% \jOneFC{The efficient processing of SPEED's custom vector instructions hinges on the underlying micro-architecture, which is meticulously designed to support these instructions and enhance the overall MP-DNN inference performance.}
%\jOneFC{The performance of SPEED's customized vector instructions relies on its micro-architecture, which is designed to efficiently support these instructions and enhance the overall MP-DNN inference performance.}
\WX{The detailed SPEED micro-architecture is shown in Fig.~\ref{fig:micro_arichi}, containing a \ding{202}~vector instruction decode unit (VIDU), a vector instruction sequencer (VIS), a \ding{203}~vector load unit (VLDU), a vector store unit, and multiple parallel computing \ding{204}~lanes, which can efficiently support customized vector instructions to enhance the overall MP-DNN inference performance.} 
%\WX{SPEED’s micro-architecture is introduced to efficiently support customized vector instructions, enhancing the overall MP-DNN inference performance.}
%\jOneFC{Fig.~\ref{fig:micro_arichi} shows the detailed micro-architecture of SPEED, embracing a \ding{202}~vector instruction decode unit (VIDU), a vector instruction sequencer (VIS), a \ding{203}~vector load unit (VLDU), a vector store unit, and multiple parallel computing \ding{204}~lanes.}
% This extension increases the dimension of parallelism, and shares storage space between tensor units and vector units, thereby improving the utilization of on-chip memory and enhancing the opportunity for data reuse.
% Based on the above considerations, this work incorporates a parameterized MPTU to the scalable module of a vector processor to achieve efficient inference for DNNs.
% The overall architecture of the vector processor will be described as follows.
% \textbf{Hardware Architecture.} 
% The detailed micro-architecture of SPEED is shown in Fig.~\ref{fig:micro_arichi}.
% To effectively handle the proposed customized vector instructions, a scalable vector processor is proposed, whose micro-architecture is shown in Fig.~\ref{fig:micro_arichi}. 

\WX{Specifically, \ding{202}~VIDU is developed to decode all vector instructions for efficient MP-DNN inference, which involves official RVV and customized vector instructions.} 
The decoded instructions are subsequently sent to the corresponding functional unit by VIS.
% Moreover, \ding{203}~VLDU is designed to facilitate two data distribution modes: sequentially transferring or multi-broadcasting data from the external memory to the scalable modules. 
\jOneFC{Additionally, \ding{203}~VLDU enables efficient data movement, offering sequential transfer and multi-broadcast capabilities from external memory to scalable modules.}
\WX{The multi-mode VLDU design allows our SPEED processor to meet the requirements of diverse data reuse patterns for various operators.}
%The multi-mode VLDU design enables our SPEED processor to meet the diverse data reuse patterns of various operators.
% The design approach enables our processor to meet the diverse computation-storage requirements of various operators.
Moreover, the scalable modules of SPEED, namely \ding{204}~lane, serve as the main computational components.
% SPEED can be configured with a variable number of identical modules, namely \ding{204}~lane, which serve as the main computational components with the architecture shown in Fig.~\ref{fig:micro_arichi}. 
% In the lane, the lane sequencer is tasked with issuing requests to read data from the Vector Register Files (VRFs) and communicating with the VIS to transmit information on the completion of instruction execution.
% Additionally, lane includes the following three units: VRFs for on-chip memory, an arithmetic logic unit (ALU) for general integer arithmetic, and a \ding{205}~parameterized multi-precision tensor unit (MPTU) dedicated to specific computation tasks.
% \jOneFC{Within each lane of SPEED's architecture, the lane sequencer is responsible for requesting data reads from the vector register files (VRFs) and notifying VIS upon completing instruction executions. 
% \jOneFC{Each lane is equipped with a lane sequencer that coordinates data flow and manages instruction execution.
% The lane also comprises three key components: the VRFs that serve as the on-chip memory, an arithmetic logic unit (ALU) for performing general integer arithmetic operations, and a parameterized multi-precision tensor unit (MPTU), which is specialized for executing specific computational tasks with high efficiency.}
\jOneFC{Each lane is equipped with a suite of components that \WX{perform} efficient data management and computation, including a lane sequencer, vector register files (VRFs), an arithmetic logic unit (ALU), and a multi-precision tensor unit (MPTU).
The lane sequencer is responsible for requesting data reads from VRFs and responding to VIS upon completing instruction executions.
% The VRFs serve as the on-chip memory, providing rapid access to data.
The VRFs within each lane serve as the local memory, enabling rapid access to data involved in computations.
The ALU performs general arithmetic operations\WX{, while the proposed MPTU focuses on} executing computation-intensive multi-precision tensor operations of MP-DNNs with high efficiency.}
%while the proposed MPTU is dedicated to executing computation-intensive multi-precision tensor operations of MP-DNNs with high efficiency.}

% \textbf{Hierarchical structure of MPTU.} 
\subsection{Hierarchical Structure of MPTU}
% To achieve efficient multi-precision data parallel processing and fully exploit data reuse opportunities, a highly flexible and parameterized MPTU is presented as the main computing unit within the lane, which is composed of three components: operand requester, queues, and tensor core.
\jOneFC{To achieve efficient multi-precision parallel data processing and maximize data reuse, a highly flexible and parameterized MPTU is incorporated into SPEED's lane as the core computing element, which comprises an operand requester, queues, and a tensor core.}
The operand requester consists of an address generator and a request arbiter, enabling efficient operand access by concurrently generating addresses and prioritizing operand requests. 
The queues are responsible for buffering the operands obtained through operand requests, including inputs, weights, accumulation data, and results.
\begin{figure}[!htp]
    \centering
    \includegraphics[width=\columnwidth]{figures/SA_core_Archi_0105.pdf}
    % \caption{Hierarchical structure of multi-precision tensor core: (a)-(c) show exapmles on how multi-precision calculations perform at 16-bit, 8-bit and 4-bit, respectively. Additionally, parallelisms which employed by tensor core are presented.}
    \caption{\jOneFC{Hierarchical architecture of multi-precision tensor core and exploited data parallelisms under (a) 16-bit, (b) 8-bit, and (c) 4-bit data precision, respectively.}}
    \label{fig:mult_precision_SA}
\end{figure}
% The tensor core serves as a critical unit to satisfy intensive computational requirements and is composed of a 2-dimensional Processing Element (PE) array, with its size determined by the parameters \#TILE\_R and \#TILE\_C.

% \rOneCN{Notably, the tensor core is a reconfigurable two-dimensional array of homogeneous processing elements (PEs) determined by the parameters \#TILE\_R and \#TILE\_C, which serves as a critical unit to flexibly satisfy the throughput requirements of various applications.}
\jOneFC{The tensor core is a two-dimensional array of processing elements (PEs) configurable by \#TILE\_R and \#TILE\_C parameters, which is designed to adapt to the throughput requirements of diverse MP-DNN applications.}
As illustrated in Fig.~\ref{fig:mult_precision_SA}, the tensor core employs an output-stationary reuse strategy, \WX{which maximizes opportunities for reusing inputs and weights.}
%which achieves high inputs and weights reuse opportunities.
% The state of the tensor core determines whether the 32-bit output is temporarily stored within the PE or shifted out across horizontal PEs to the result queue.
\WX{The decision of whether to temporarily retain the 32-bit output within the PE or transfer it horizontally to the result queue depends on the tensor core's state, specifically, the completion of the current computation.}
%\rThreeCN{The state of the tensor core determines whether the 32-bit output is to be temporarily retained within the PE or transferred horizontally to the result queue, depending on the completion of the current computation.}
% As illustrated in Fig.~\ref{fig:mult_precision_SA}, the tensor core employs an output-stationary reuse strategy and works in a pipeline manner.
% This design enables the tensor core to fully reuse data, achieving high computational throughput without increasing storage space.
% During the computation, each PE reads the weights (inputs) from up (left) and transfers the weights (inputs) to down (right), while also accumulating the product of the inputs and weights.
\WX{Each PE stores the incoming data in an internal register and forwards the same data to its neighbor PE.
These store and forward behaviors contribute to significant savings in external memory accesses, effectively exploiting data reuse opportunities.}
As depicted in Fig.~\ref{fig:mult_precision_SA}, the proposed PE contains sixteen 4-bit multipliers, which can perform one set of 16-bit multiply-accumulate (MAC) \WX{operations}, four sets of 8-bit MAC operations, and sixteen sets of 4-bit MAC operations.

% The state of tensor core determines whether the 32-bit output is temporarily stored within the PE or shifted out across horizontal PEs to the result queue.
% \rOneCN{Waiting for modified!!!}
Fig.~\ref{fig:mult_precision_SA} shows that tensor core architecture employs three levels of parallelism, \WX{denoted by} parallelism within PE ($PP$), parallelism on inputs ($POI$), and parallelism on weights ($POW$). 
The value of $PP$ depends on the operand precision. For 16-bit, 8-bit, and 4-bit operands, $PP$ is 1, 4, and 16, respectively.
Meanwhile, the values of $POI$ and $POW$ are determined by the size of the tensor core, i.e., \#TILE\_R and \#TILE\_C.
%补一下如何根据网络尺寸分配并行度
% 太抽象了，还是放到dataflow那边去写
% In multi-dimensional array computations, the PP is often performed on dimensions requiring adjacent computations to fully leveraging data reuse opportunities offered by overlapping data, such as the row dimension of the left matrix, the column dimension of the right matrix in MM, as well as the input channel dimension in CONV.
% To further improve computing efficiency, POI and POW are utilized for parallel processing along dimensions without data dependency.
% For instance, in MM, the POI row vectors of the left matrix can be partitioned into groups, and the MAC operation of each row vector with the POW column vectors of the right matrix can be performed in parallel.}
% In matrix computation, parallelism in the row and column dimensions of the left matrix are POI and PP, respectively, and parallelism in the row and column dimensions of the right matrix are determined by PP and POW.
% For convolution computation, PP is implemented in the input channel dimension, while POI and POW are employed in the feature map and output channel dimensions, respectively.
% \rTwoCN{\textbf{New version begins:}}
% In multi-dimensional array computations, PP is proposed to fully leverage data reuse opportunities provided
% by overlapping data between adjacent computations.
\WX{The parallel computation within PE is implemented to minimize the extra data movement provided by overlapping data between adjacent computations, fully leveraging data reuse opportunities.
The parallel computing data for inputs and weights are arranged in an orthogonal pattern to align with the structure of the multi-dimensional array, significantly enhancing the computational efficiency of the MPTU.}
%%$PP$ is proposed to minimize the extra data movement provided by overlapping data between adjacent computations occurring within the same PE, thereby fully leveraging data reuse opportunities.
% POI and POW are strategically employed for parallel processing across various dimensions, enabling direct matrix-matrix computations and further enhancing the computational efficiency of the MPTU.
%\rThreeCN{$POI$ and $POW$ are arranged in an orthogonal pattern that aligns with the structure of multi-dimensional array computations, facilitating parallel processing along independent dimensions and further enhancing the computational efficiency of the MPTU.}
% Furthermore, the three levels of parallelism allow for a versatile data mapping approach, offering adaptability for various operators, as detailed in Sec.~\ref{sec: dataflow_design}.
\WX{Moreover, utilizing these three levels of parallelism can offer a flexible dataflow mapping opportunity, enabling the tensor core with high computational efficiency for various MP-DNN  operators, which is elaborated in Sec.~\ref{sec: dataflow_design}.}
%\jOneFC{The three levels of exploited parallelism offer a flexible dataflow mapping opportunity, enabling the tensor core with high computational efficiency for various MP-DNN operators, which is elaborated in Sec.~\ref{sec: dataflow_design}.}


% \rTwoCN{\textbf{New version ends}}

% MPTU can flexibly compatible with the parallel dimension requirements of different tensor computation operators, achieving higher computational efficiency with fewer storage resources and thereby enabling efficient inference for multi-precision DNNs.
% \rOneCN{ 
% The MPTU increases the parallelism dimensions of the scalable modules and provides a more flexible method for adjusting parallelism, making it more suitable for handling multi-dimensional array computations with different throughput requirements. 
% Additionally, the MPTU enhances data reuse opportunities, achieving efficient DNN inference with minimal area overhead.}
% \section{The Mixed Dataflow Architecture in Hardware}\label{sec: dataflow_design}
\section{The Proposed Flexible Mixed Dataflow}\label{sec: dataflow_design}
% The section introduces a mixed dataflow architecture optimized for both matrix and convolution computations, aiming to enhance computational efficiency and data utilization. 
% The architecture supports rapid configuration of dataflow strategies through a single \texttt{VSACFG} instruction, holding the potential for efficient inference of various DNN workloads.
% The design and implement details of matrix dataflow strategy and three convolution dataflow strategies in the architecture are discussed below.
\WX{
%The section introduces a flexible mixed dataflow mapping method in collaboration with the \texttt{VSACFG} configuration instruction to optimize the computing data arrangement.
%Specifically, we propose a matrix multiplication dataflow strategy for the MM operator, along with FFCS, CF, and FF strategies for the CONV, PWCV, and DWCV operators, respectively.
% The section introduces a flexible mixed dataflow mapping method in collaboration with the \texttt{VSACFG} configuration instruction to optimize the computing data arrangement, consisting of a matrix multiplication dataflow strategy for the MM operator, along with FFCS, CF, and FF strategies for the CONV, PWCV, and DWCV operators, respectively.
\jOneFC{This section elaborates on the proposed flexible mixed dataflow mapping method, which aims to optimize the data arrangement for MP-DNN computing.}
\jOneFC{It consists of a matrix multiplication dataflow strategy for the MM operator, along with Feature-Map-First-Channel-Second~(FFCS), Channel-First~(CF), and Feature-Map-First~(FF) strategies for the CONV, PWCV, and DWCV operators, respectively.}
These strategies fully exploit data reuse opportunities brought by these operators and computation parallelism in SPEED, further improving MP-DNN deployment performance.
}
% These dataflow strategies include Feature-Map-First-Channel-Second~(FFCS) for CONV operator, Channel-First~(CF) for PWCV operator, and Feature-Map-First~(FF) for DWCV operator.
% \WX{The section introduces a flexible mixed dataflow mapping method in collaboration with the \texttt{VSACFG} configuration instruction to optimize the computing data arrangement for different operators, including MM, CONV, PWCV, and DWCV, which fully exploits data reuse opportunities brought by these operators and computation parallelism in SPEED, further improving MP-DNN deployment performance.}
%significantly enhancing computational efficiency.
%%%%%%%%%%%%%%%%%%%%%%%
% \rOneCN{
% The section introduces a flexible mixed dataflow mapping method with rapid configuration empowered by the \texttt{VSACFG} instruction, and optimizes the dataflow strategies for different computation-storage density characteristic operators, including MM, CONV, PWCV, and DWCV, aiming to enhance computational efficiency.
% Furthermore, these dataflow strategies fully exploits data reuse opportunities provided by accumulating data between adjacent computations and multi-broadcasting data across the scalable modules.
% Furthermore, these dataflow strategies fully exploit the hierarchical parallelism provided by the processor and achieve high data reuse opportunities through efficient data arrangement.
% Detailed descriptions of the mixed dataflow mapping method are provided below.
% }
%%%%%%%%%%%%%%%%%
\begin{figure*}[!htbp]
  \centering
    \includegraphics[width=2\columnwidth]{figures/matu_dataflow.pdf}
      \caption{\WX{An example of computing dataflow strategy for 8-bit MM operators. }}
      % Note that the 16-bit and 4-bit MM follow a similar method, with differences in computation parallelism.}}
        \label{fig:matu_dataflow}
\end{figure*}

%An example of executing dataflow in 8-bit matrix computation is explained in detail. Note that the 16-bit and 4-bit matrix computations are operated in the same way but with different PP.
\subsection{Matrix Multiplication Dataflow Strategy}\label{sec: matrix_dataflow}
% To enhance the efficiency of matrix multiplication computations in DNNs, especially those with transformer structures, based on the parallel processing capability of MPTU, a matrix dataflow strategy is proposed that exploits matrix operands in parallel from multiple dimensions and significantly improve computation efficiency. 
\WX{MM is a fundamental operation that forms the core computation within Transformer. 
Additionally, convolution operations can be converted into MM operators for efficient processing. 
Thus, optimizing \jOneFC{the scheduling of MM operators} becomes crucial for improving the performance of MP-DNN deployments.}
% \jOneFC{Exploring the dataflow scheduling of MM operators is crucial for improving the performance of MP-DNN deployments, as }
% \WX{However, due to the limited three computation loops, MM offers limited data reuse opportunities and computation parallelism.}
\jOneFC{Limited by its three computation loops, the MM operator suffers from restricted data reuse and parallelism.}
%hardware design faces constraints in terms of data parallel dimensions and data reuse opportunities.
\WX{To solve this issue, we propose an efficient MM dataflow strategy to perform the parallel MM execution.}
\jOneFC{Specifically, it leverages multi-broadcasting of weights across scalable modules and input reuse across processing stages, optimizing the arrangement of parallel computing data and achieving significant gains in computational efficiency.}
% Specifically, it multi-broadcast weights among scalable modules and reuses inputs in multiple processing stages to optimize the arrangement of parallel computing data, significantly enhancing computational efficiency.

\WX{To elaborate on the proposed MM dataflow strategy, we take the four processing stages of 8-bit MM operators as an example, depicted in Fig.~\ref{fig:matu_dataflow}.}
\WX{The processor is configured with two lanes, where each lane is equipped with a tensor core of size 2$\times$2 to satisfy the requirements of parallel computations ($POI$ = $POW$ = 2).
Within each lane, the data in $POI$ adjacent rows of the left matrix are multiplied simultaneously with those in $POW$ adjacent columns. Additionally, $PP$ data from adjacent computations are processed in the same PE to fully exploit the parallelism provided by MPTU.
}
%where the size of the tensor core in each lane is set as 2$\times$2 to satisfy the requirements of parallel computations ($POI$ = $POW$ = 2).

%\rTwoCN{
%To achieve efficient deployment of MM, a matrix dataflow strategy is proposed that implements parallel processing in multiple dimensions and achieves high data reuse.
%The matrix dataflow strategy, with its optimized parallelism arrangement, significantly enhances computational efficiency.
%Furthermore, the strategy achieves sufficient data reuse opportunities by multi-broadcasting weights between scalable modules and reusing inputs in multiple stages.}
%补充MM数据流的优势
%To elaborate on the benefits of the matrix dataflow strategy, Fig.~\ref{fig:matu_dataflow} illustrates the four processing stages of 8-bit matrix computation as an example to discuss the details. 
%\rTwoCN{
%Within each lane, POI adjacent rows of the left matrix are multiplied with POW adjacent columns in parallel.
%Meanwhile, the PP provided by MPTU is fully exploited by arranging the dataflow of adjacent computations on the same PE.
% Within each lane, the product of POI row vectors of the left matrix and POW column vectors of the right matrix are computed in parallel. 
% Meanwhile, the PP provided by MPTU is fully exploited by arranging the dataflow of adjacent computations on the same PE. }
% The parallelism of the left and right matrices in the column and row dimensions, respectively, is PP, which means that every four adjacent operands are processed by the same PE.
%In the context of 8-bit computations, the PP value is 4.
%Concurrently, we configure the processor with two lanes, and the size of the tensor core in each lane is 2$\times$2, which means both POI and POW are 2.
%}

\WX{
As shown in Fig.~\ref{fig:matu_dataflow}, the input queue and weight queue of each lane send computing data to PEs, where the results are organized in the result queue and subsequently stored in the VRFs.
%, while the results are organized in the result queue and subsequently stored in the VRFs. 
Considering the $PP$ is set as 4 in 8-bit computations, four neighbouring data of the computation matrix are combined as a single operand, such as inputs~\ding{192}. 
% \rFourCN{Additionally, in 4-bit computations, with $PP$ set to 16, a single operand within the computation matrix is composed of sixteen adjacent data.}
%Specifically, 
In the first stage, inputs \ding{192}, \ding{194} and \ding{196}, \ding{198} are allocated to two lanes, respectively, with each lane reusing the same weights \Rmnum{1} and \Rmnum{3}. 
The weight queue requests weights \Rmnum{5} and \Rmnum{7} for the next stage, while the same data in the input queue are reused in PEs to perform computations along the row dimension of the right matrix.
%, while the same data in the input queue are reused to perform computations along the row dimension of the right matrix. 
In the third stage, the input queue fetches new data (inputs \ding{193}, \ding{195} and \ding{197}, \ding{199}) along the rows of the left matrix for computation in each lane by reusing weights \Rmnum{2} and \Rmnum{4}. 
Besides, the results generated in the first stage, temporarily buffered in the accumulation queue to reduce the off-chip data transfer, are requested from the VRFs during the computation process. 
They are added to the results of the current stage to obtain output results. 
Similarly, in the fourth stage, the same data in the input queue from the previous stage are multiplied by their corresponding weights \Rmnum{6} and \Rmnum{8}. 
The results are accumulated with the partial sum from the second stage to complete the computation of one row in the output matrix.}
%The input queue and weight queue of each lane send computing data to PEs, while the results are organized in the result queue and subsequently stored at the VRFs. Specifically, in the first stage, inputs 1, 3 and inputs 5, 7 are allocated to two lanes, respectively, with each lane reusing the same weights I and III. The weight queue requests weights V and VII in the next stage, while the data in the input queue are reused to perform computations along the row dimension of the right matrix. In the third stage, the input queue fetches new data (inputs 2, 4 and inputs 6, 8) along the rows of the left matrix, and weights II and IV are broadcasted to the same lanes. The results generated in the first stage, temporarily buffered in the accumulation queue to reduce the off-chip data transfer, are requested from the VRFs during the computation process. They are added to the results of the current stage to obtain complete output results. These operations are repeated in the fourth stage, multiplying the data in the input queue of the previous stage with their corresponding weights VI and VIII. The results are accumulated with the partial sum from the second stage to complete the computation of one row in the output matrix.

%At the first stage, inputs~\ding{192} ,~\ding{194} and ~\ding{196} ,~\ding{198} are sequentially allocated to two lanes, each lane utilizing the same weights \Rmnum{1} and \Rmnum{3} for high data reuse. 
%The input queue and weight queue of each lane distribute operands to the PEs for parallel computation. 
%The results are placed in the result queue, and then stored at the VRFs.
%To enhance data reuse and on-chip storage utilization, operands in the input queue are reused in the second stage, while the weight queue request weights \Rmnum{5} and \Rmnum{7} from the right matrix along the row dimension for computation.
%In the third stage, the input queue fetches new operands (inputs~\ding{193} ,~\ding{195} and ~\ding{197} ,~\ding{199}) along the rows of the left matrix, and weights \Rmnum{2} and \Rmnum{4} are broadcasted to both lanes for computation. 
%For decreasing the DRAM access size and data transmission delay, the results of the first stage are requested from VRFs and buffered in the accumulation queue during the computation process, and then add to the results of current stage for obtaining part of the output matrix operands.
%The operations are repeated in the fourth stage, utilizing the operands in the input queue of the previous stage and corresponding new weights \Rmnum{6} and \Rmnum{8} for computation. 
%The result are accumulated with the partial sum from the second stage to get the another part operands of the output matrix.


\subsection{Convolution Dataflow Strategy}\label{subsec: conv_dataflow}
% \WX{Convolution, as a pivotal operation in CNN models, plays a crucial role in network execution.
% Recently, in pursuit of higher performance, convolutional variants like DWCV and PWCV have been developed to satisfy the demands of various tasks. 
% However, due to distinct computing and storage characteristics exhibited by these operations, simply employing a unified dataflow strategy to execute them would lead to an unacceptable degradation in computational utilization.
\jOneFC{Convolution operators are critical for the performance of CNNs.
% \jOneFC{and recent developments like DWCV and PWCV cater to diverse tasks.
\WX{In pursuit of higher performance, convolutional variants like DWCV and PWCV have been developed to satisfy the demands of various tasks on top of CONV.}
However, their unique computational and storage needs mean that a one-size-fits-all dataflow approach would suffer from under-utilized computation.}
\WX{To solve this issue, we propose multiple dataflow strategies towards varied CNN operators for efficient inference of MP-DNNs.}
% \jOneFC{These dataflow strategies include Feature-Map-First-Channel-Second~(FFCS) for CONV operator, Channel-First~(CF) for PWCV operator, and Feature-Map-First~(FF) for DWCV operator.}
\rFourCN{These dataflow strategies include FFCS for CONV operator, CF for PWCV operator, and FF for DWCV operator.}
% \WX{Specifically, these strategies, namely Feature-Map-First-Channel-Second~(FFCS), Channel-First~(CF), and Feature-Map-First~(FF), are designed to optimize CONV, PWCV, and DWCV computations, respectively.}
%as another main operation of DNNs, dominates the execution in CNN models. 


%To achieve efficient inference for multi-precision DNNs, which consist of various operators with different computation-storage density requirements, a mixed dataflow strategy for convolution computations is proposed to compatible with CONV, PWCV and DWCV operators.
%The mixed dataflow strategy includes three dataflow strategies: Feature map First Channel Second~(FFCS), Channel First~(CF), and Feature map First~(FF). 
%Among them, FFCS is suitable for CONV computations, CF for PWCV computations, and FF for DWCV computations. 

\WX{To provide a detailed explanation of the proposed convolution dataflow strategies, we take the four processing stages of 16-bit 3$\times$3 convolution computations as an example. 
Fig.~\ref{fig:conv_dataflow} depicts the data pre-fetch of 16-bit inputs (X16) and 16-bit  weights (W16), as well as the data arrangement within the lane. 
In the case of 16-bit parallel computations, we set $POI$, $POW$, and $PP$ to 2, 2, and 1, respectively. 
In Fig.~\ref{fig:conv_dataflow}~(a), the upper part displays the pre-fetched data of the X16 input feature map (Fmap) for the four processing stages, with different dataflow strategies represented by the data inside the green dotted line (FFCS), blue dashed line (CF), and red solid line (FF). 
The lower part of Fig.~\ref{fig:conv_dataflow}~(a) illustrates the corresponding W16 kernel Fmap for four stages.}


%To elaborate on the proposed convolution dataflow strategies, we take the four processing stages of 16-bit 3$\times$3 convolution computations as an example, with the descriptions of data pre-fetch of 16-bit inputs (X16) and 16-bit  weights (W16) and the data arrangement within the lane depicted in Fig.~\ref{fig:conv_dataflow}. 
%For 16-bit parallel computations, $POI$, $POW$, and $PP$ are set to 2, 2, and 1. 
%The upper part of Fig.~\ref{fig:conv_dataflow}~(a) shows the pre-fetched data of the X16 input feature map (Fmap) for different dataflow strategies in the four processing stages, where the data inside the green dotted line, blue pecked line, and red solid line are on behalf of the prefetched data for the FFCS, CF, and FF strategies, respectively. 
%The lower part illustrates the corresponding W16 kernel Fmap for four stages.

%%%%%%%%%%%%%
%To illustrate the working principles of different convolution dataflow strategies clearly, the first four processing stages of 16-bit convolution computations are selected for analysis, showing the data pre-fetch of 16-bit inputs (X16) and 16-bit weights (W16) and the data arrangement within the lane. 
%As depicted in Fig.~\ref{fig:conv_dataflow}, the weight kernel size is 3$\times$3, with $POI$ and $POW$ values both set to 2, and $PP$ is 1 due to 16-bit computations.
%The upper part of Fig.~\ref{fig:conv_dataflow}~(a) shows the pre-fetched data in the four processing stages of the X16 input feature map (Fmap) for three different dataflow strategies.
%Specifically, the data inside the dotted line, pecked line, and solid line correspond to the prefetched data for the FFCS, CF, and FF strategies, respectively. 
%The lower part illustrates the corresponding W16 kernel fmap for four stages.  
%%%%%%%%%
% These three dataflows are detailed in the subsequent sections.
% Specifically, the data inside the green box, blue box, and brown box correspond to the prefetched data for the FFCS, CF, and FF strategies, respectively. 

% \begin{figure*}[!htbp]
%   \centering
%     \includegraphics[width=2\columnwidth]{figures/conv_dataflow.pdf}
%       \caption{
%       \WX{Three convolution dataflow strategies of SPEED for supporting different convolutional operators: (a) data pre-fetch of input Fmap and weight kernel Fmap, (b) multiple sets of inputs and weights for a complete convolution operation. (c)-(e) are examples of computing dataflow of three convolution dataflow strategies, where the same inputs and the weights are sent to different lanes.}
%       % Note that the 8-bit and 4-bit convolution computations are operated similarly except for the parallelism value.}
%      }
%         \label{fig:conv_dataflow}
% \end{figure*}

\begin{figure}[htbp]
  \centering
    \includegraphics[width=1\columnwidth]{figures/conv_dataflow_1.pdf}
      % \caption{FF vs. CF and mi$\times$ strategies layer-wise performance for GoogleNet.}
      % \caption{Performance result comparisons between Ara and different dataflow strategies under various kernel-size configurations.}
      \caption{Prefetching and partitioning of input Fmap and weight kernel Fmap: (a) data pre-fetch of input Fmap and weight kernel Fmap, (b) multiple sets of inputs and weights for a complete convolution operation. }
    \label{fig:conv_dataflow_1}
    \vspace{-0.8em}
\end{figure}

\begin{figure}[htbp]
  \centering
    \includegraphics[width=1\columnwidth]{figures/conv_dataflow_2.pdf}
      % \caption{FF vs. CF and mi$\times$ strategies layer-wise performance for GoogleNet.}
      % \caption{Performance result comparisons between Ara and different dataflow strategies under various kernel-size configurations.}
      \caption{Three convolution dataflow strategies of SPEED for supporting different convolutional operators: (a)-(c) are examples of computing dataflow of three convolution dataflow strategies, where the same inputs and the weights are sent to different lanes.}
    \label{fig:conv_dataflow_2}
    \vspace{-0.8em}
\end{figure}

%An example of mapping three convolution dataflow strategies to hardware architecture. (a) data pre-fetch of input feature map (Fmap) and weight kernel Fmap, (b) mutiple sets of inputs and weights for a complete convolution operation, (c)-(e) examples of computing dataflow in three convolution dataflow strategies, where the same inputs are sent to different lanes and the weights are distributed orderly to different lanes. Note that the 8-bit and 4-bit convolution computations are operated in the same way but with different $PP$.

\WX{Fig.~\ref{fig:conv_dataflow}~(b) illustrates multiple sets of inputs and weights for the FFCS, CF, and FF strategies during the convolution computation stages. 
Each set provides the operands required for parallel convolution computations. 
For instance, the inputs \ding{192}--\ding{195} are organized by traversing the 3$\times$3 convolution window in the first input channel of $I_{0}$, while inputs \ding{196}, \ding{197}, and \ding{198}, \ding{199} are organized from other input channels of $I_{0}$, respectively. 
Regarding the weights, $K_0$ and $K_1$ are combined along the input channel dimension to generate four sets of weights, and $K_2$ and $K_3$ follow a similar manner. 
In each stage, the same inputs are sent to two lanes, while weights of different output channels are distributed to specific lanes. 
Besides, as previously mentioned, three levels of parallelism computations are implemented in SPEED. 
The parallelism in the input channel dimension for inputs and weights is determined by $PP$, with $PP$ set as 1, 4, and 16 for 16-bit, 8-bit, and 4-bit operands, respectively. 
The parallelisms in the feature map and output channel dimensions are determined by $POI$ and $POW$, respectively.}

%please help me refine the sentence: Multiple sets of inputs and weights for FFCS, CF, and FF strategies in the convolution computation stages are depicted in Fig. 6 (b), where each set provides the operands required for parallel convolution computations. For instance, the inputs ➀–➃ are organized by traversing the 3×3 convolution window in the first input channel of I0, while inputs➄, ➅, and ➆, ➇ are organized from other input channels of I0, respectively. For weights, K0 and K1 are combined along the input channel dimension to generate four sets of weights. K2 and K3 can be obtained similarly. In each stage, the same inputs are sent to two lanes, while weights of different output channels are distributed to certain lanes. Besides, as mentioned before, three levels of parallelism computations are implemented in SPEED. Specifically, the parallelism in the input channel dimension for inputs and weights is determined by PP, with PP set as 1,4 and 16 for 16-bit, 8-bit  and 4-bit operands, respectively. The parallelisms in the feature map and output channel dimensions are determined by POI and POW, respectively.

%Fig.~\ref{fig:conv_dataflow}~(b) illustrates multiple sets of inputs and weights for FFCS, CF, and FF strategies in the convolution computation stages. 
%Each set of inputs and weights provide the operands required for parallel processing of $POI$ and $POW$ complete convolution computations, respectively.
%\rThreeCN{The \ding{192}--\ding{195} of $I_{0}$ are obtained by traversing the 3$\times$3 convolution window on the first input channel, while \ding{196}--\ding{197}, \ding{198} and \ding{199} belong to the other three input channels of $I_{0}$, respectively.}
% The \ding{192}--\ding{195} of $I_{0}$ are obtained by traversing operands on the first input channel, while \ding{196}--\ding{197}, \ding{198} and \ding{199} belong to the other three input channels of $I_{0}$, respectively.
%$K_0$ and $K_1$ are combined according to different input channels, resulting in four sets of weights. $K_2$ and $K_3$ are operated in the same way.
% in each stage
%In each stage, the same inputs are sent to different lanes, and weights located in different output channels are distributed to the corresponding lanes.
%Base on the data allocation of each stage, all dataflow strategies empoly three levels of parallelism.
% : lanes$\times$POW in the output channel dimension, POI in the feature map dimension, PP in the input channel dimension.
%The parallelism in the input channel dimension for inputs and weights is $PP$, with $PP$ values of 1,4 and 16 for 16-bit, 8-bit and 4-bit operands, respectively.
%The other two parallelisms, $POI$ and $POW$, are applied in the feature map and output channel dimensions, respectively. 

\WX{Fig.~\ref{fig:conv_dataflow}~(c) shows the data arrangement across stages for the three dataflow mapping strategies, where the operations can be classified into two categories: operation 1 (OP1) and operation 2 (OP2). 
In OP1, the inputs are traversed along the feature map dimension, utilizing the same weights as in the previous stage. 
In OP2, new inputs and weights are requested along the input channel dimension. 
The computation process for these strategies is elaborated as followings.}

%In order to clearly illustrate the differences in data arrangement across stages among the three dataflow strategies, as shown in Fig.~\ref{fig:conv_dataflow}~(c), the operations between stages are divided based on dimensions: operation 1 (OP1) and operation 2 (OP2).
%In OP1, the inputs are traversed along the feature map dimension, while reusing the weights from the previous stage.
%In OP2, the inputs and weights are requested along the input channel dimension.
%The computation process of three dataflow strategies are explained in detail below.

\textbf{FFCS strategy.}
\WX{The data arrangement for the FFCS strategy involves multiple computation stages, denoted as ``N stages'' in Fig.~\ref{fig:conv_dataflow}~(c). 
%Within these stages, OP1 is executed to fully utilize the data reuse opportunities by multiplying inputs with the same weights. 
%After completing the N-th stage, OP2 is performed to request data along the input channel dimension, relieving the storage pressure on VRFs. 
%In the subsequent N stages, OP1 is repeated across stages, where the results of the latter N stages are accumulated with the partial sum obtained in the former N stages to reduce off-chip DRAM access.
Within these stages, SPEED executes OP1 to fully utilize the data reuse opportunities by multiplying inputs with the same weights.
After completing the N-th stage, SPEED performs OP2 to request data along the input channel dimension, relieving the storage pressure on VRFs.
In the subsequent N stages, SPEED repeats OP1 across stages, where the results of the latter N stages are accumulated with the partial sum obtained in the former N stages to reduce off-chip DRAM access.}

\WX{For example, in the case of N=2, inputs $I_{0}$--\ding{192} are multiplied with weights $K_{0}\&K_{1}$--\ding{192} and $K_{2}\&K_{3}$--\ding{192} in the first stage, while the weights are reused by $I_{0}$--\ding{193} in the next stage. 
In the third stage, inputs are traversed from the second input channel of $I_{0}$ and computed with the weights $K_{0}\&K_{1}$--\ding{193}, and $K_{2}\&K_{3}$--\ding{193}, respectively. 
Besides, the partial sums obtained in the first stage are requested from the VRFs and buffered in the accumulation queue, awaiting addition to the result of the current stage. 
Note that the partial sums of the third stage are stored in the same address as those of the first stage in the VRFs to minimize on-chip storage consumption. 
In the fourth stage, the weights of the previous stage are reused to perform convolution computations with $I_{0}$--\ding{197}. 
Subsequently, the current computation results are accumulated with the partial sums obtained in the second stage, and the results are stored back in the VRFs after the accumulation.}

%The FFCS strategy utilizes OP1 between N stages, the repeated usage of the same weights improving the data reuse opportunities.
%After the N-th stage, OP2 is employed, requesting data along the input channel direction for decreasing the foot-print of VRFs, and OP1 is used in the subsequent N stages for high data reuse.
%The results of the latter N stages are accumulated with the partial sum of the former N stages, reducing on-chip storage space occupancy and access size of off-chip DRAM. 
%As depicted in Fig.~\ref{fig:conv_dataflow}~(c), in the following instance, N set to 2.
%In the first stage, inputs $I_{0}$--\ding{192} are computed with weights $K_{0}\&K_{1}$--\ding{192} and $K_{2}\&K_{3}$--\ding{192}, and the results are output after the computation.
%Weights are reused in the second stage and operated with $I_{0}$--\ding{193}.
%In the third stage of FFCS, inputs are traversed from the second input channel of $I_{0}$, and computed with the corresponding weights $K_{0}\&K_{1}$--\ding{193}, $K_{2}\&K_{3}$--\ding{193}, respectively.
%During the computation, the partial sums of the first stage are requested from the VRFs and buffered in the accumulation queue, waiting to be added to the result of the current stage.
%To reduce the consumption of on-chip storage, the storage address of the partial sum from the third stage in the VRFs is the same as that of the first stage.
%The fourth stage also reuses the weight of the previous stage and performs convolution computations with $I_{0}$--\ding{197}.
%Simultaneously, the partial sums of the second stage are retrieved and accumulated with the current computation results. 
%The results are stored back in the VRFs after the accumulation.

\textbf{CF strategy.}
% \WX{For PWCV, VRF accesses required in the FFCS strategy would cause significant time wastage in transmitting partial results accounting for a large portion of the whole computation time since the convolution kernel size is too small.}
\jOneFC{PWCV operators are poorly suited for the FFCS strategy. The small convolution kernel size necessitates frequent VRF accesses for partial results, leading to significant data transmission overhead that dominates the overall computation time.}
\WX{To address this issue, SPEED employs the CF strategy to traverse along the input channel dimension firstly among stages, allowing for the accumulation of partial sums within the PE to eliminate extra data transmissions between MPTU and VRFs.
As depicted in Fig.~\ref{fig:conv_dataflow}~(d), in the first stage, the inputs from the first input channel, $I_{0}$--\ding{192}, are multiplied by weights $K_{0}\&K_{1}$--\ding{192} and $K_{2}\&K_{3}$--\ding{192}, where the results are stored in PEs. 
In the subsequent three stages, the inputs from the 2nd, 3rd, and 4th input channels of $I_{0}$ are performed with their corresponding weights. 
Besides, the computed results are consumed by adding to the partial sums previously stored in PE for the generation of a complete output, which continues until all input channels have been traversed. 
The final outputs are stored in the VRFs via the result queue.}

%When dealing with convolution computations with low data reuse requirements, FFCS strategy excessively accesses VRFs, leading to extra time consumption in transferring the partial results. 
%In order to avoid output transfer latency, the CF strategy that traverses along the input channel between stages is proposed.
%The CF strategy utilizes the output stationary feature of the tensor core and performs partial sum accumulation within the PE, avoiding multiple data transmission between MPTU and VRFs, thereby improving computational efficiency.
%In the first stage, $I_{0}$--\ding{192} of the first input channel is computed with $K_{0}\&K_{1}$--\ding{192} and $K_{2}\&K_{3}$--\ding{192} respectively, and the results are saved in PE.
%In the following three stages, the inputs on the 2nd, 3rd and 4th input channels of $I_{0}$ are convolved with the corresponding weights, and the results are added to the partial sums stored in PE for enhancing data utilization.
%The accumulation repeats until all input channels are processed and then results are stored in the VRFs through the result queue.

\textbf{FF strategy.}
\WX{For DWCV, since it decouples the dependency across different input channels, SPEED employs the FF strategy to improve computational efficiency without performing accumulation operations in the input channel dimension.
Specifically, the proposed FF strategy performs OP1 among different stages to fully exploit data reuse opportunities by traversing inputs within a single input channel with the same weights multiplied, which also reduces off-chip data accesses. 
As shown in Fig.~\ref{fig:conv_dataflow}~(e), inputs $I_{0}$--\ding{192} to $I_{0}$--\ding{195} are obtained by traversing along the first input channel of $I_{0}$, where each input performs computation with the same weights in every computation stage. 
The partial sum is sent to the VRFs through the result queue. 
The above operations are repeated in subsequent stages until the computations for a single input channel are completed.}

% The FFCS and CF strategies are optimized on the input channel dimension and are not suitable for depth-wise operations.
%\rOneCN{
%The FF strategy always exploits OP1 between various stages, which fully takes advantage of data reuse opportunities by traversing inputs on a single input channel and reusing weights, further reducing off-chip data access.
%Without performing accumulation operations on the input channel dimension, the FF strategy is suitable for depth-wise operations.}
% The FF strategy is optimized for depth-wise operations, which involves multiple data reuses on a single input channel, increasing data reuse opportunities, reducing off-chip data access, thereby improving computational efficiency, and achieving low power consumption.
%FF strategy traverses along the first input channel of $I_{0}$, obtaining $I_{0}$--\ding{192} to $I_{0}$--\ding{195}, and computes them with the same weights in each stage for decreasing DRAM access size.
%The partial sum is output to the VRFs through the result queue between each stage.
%The operations are repeated in subsequent stages until the computations for a single input channel are completed.
\begin{figure}[!htbp]
  \centering
    \includegraphics[width=1\columnwidth]{figures/dataflow_implement.pdf}
      \caption{\WX{An example of scheduling process in the first two stages of the FFCS dataflow strategy.}
       }
        \label{fig:dataflow_implement}
\end{figure}
%An example of mapping FFCS dataflow strategy to the proposed hardware architecture with customized instructions. 
\subsection{Execution Flow of Convolution Dataflow Strategy}\label{subsec: dataflow_implement}
% In the following section, to illustrate clearly how dataflow strategies are efficiently processed in hardware under instruction scheduling, we provide a detailed explanation using the deployment of the FFCS strategy for the first two stages with a convolution kernel size of 3x3 as an example.
%\rOneCN{
%To illustrate the scheduling process of dataflow strategies, we take the first two stages of the FFCS dataflow strategy as an example to introduce in detail, and provide a detailed explanation in the following section.}
%Here, the configurations are the same as in Sec.~\ref{subsec: conv_dataflow}.
% As explained in Sec.~\ref{subsec: instr_design}, the \texttt{VSACFG} configuration-setting instruction is executed in the setup stage for parameters configuration, and the \texttt{VSALD} and \texttt{VSAM} instructions are executed in the compute stage.
%\rOneCN{
%As explained in Sec.~\ref{subsec: instr_design}, the \texttt{VSACFG} configuration-setting instruction is executed during the setup stage for parameters configuration, followed by the \texttt{VSALD} and \texttt{VSAM} instructions in the compute stage.}

\WX{To illustrate the scheduling process of dataflow strategies, we provide an example in Fig.~\ref{fig:dataflow_implement}, focusing on the first two stages of the FFCS strategy, where the hardware configurations remain consistent with those described in Sec.~\ref{subsec: conv_dataflow}. 
The scheduling process is controlled by a set of instructions comprising configuration-setting, memory access, and arithmetic instructions, as detailed in Sec.~\ref{subsec: instr_design}.}

\WX{Specifically, VIDU decodes the parameters within the \texttt{VSACFG} instruction, which are subsequently sent to the functional units for 16-bit 3$\times$3 convolution computations following the FFCS strategy. 
The memory access instructions, \texttt{VSALD} and \texttt{VLE}, are responsible for loading inputs and weights, such as $I_{0}$ and $K_0$\&$K_1$, into the VRFs, which buffer computing data for continuous computations.}



%\WX{To illustrate the scheduling process of dataflow strategies, we take the first two stages of the FFCS dataflow strategy as an example in Fig.~\ref{fig:dataflow_implement}, where the hardware configurations are the same as in Sec.~\ref{subsec: conv_dataflow}.}
%The scheduling process is managed by a set of instructions that consist of configuration-setting, memory access, and arithmetic instructions, as detailed in Sec.~\ref{subsec: instr_design}. 

% 数据流的参数配置、数据调度以及计算是与一系列指令紧密配合完成的，所需的指令如同Section B所描述的那样，包括configuration-setting、memory access和arithmetic指令。
% 具体来说，
% configuration-setting指令VSACFG中包含的参数被VIDU解码并发送到各个功能单元中，以便使用FFCS strategy处理16-bit 3×3 convolution computation。
% memory access指令 \texttt{VSALD} and \texttt{VLE}分别加载inputs和weights到VRFs中，VRFs被分成了inputs、weights和accumulation三块，对应地址分别为weights memory（WMEM）、inputs memory（IMEM）和 accumulation memory（AMEM）。


%Specifically, the parameters in VSACFG  instruction are decoded by VIDU and subsequently sent to functional units for 16-bit 3$\times$3 convolution computations following the FFCS strategy. 
%The memory access instructions, VSALD and VLE, are responsible for loading inputs and weights, like $I_{0}$ and $K_0$\&$K_1$, into the VRFs.
%that buffer computing data for continuous computations.

%\rFourCN{
%The scheduling process is cooperated with a set of instructions, as detailed in Sec.~\ref{subsec: instr_design}, which consists of configuration-setting, memory access, and arithmetic instructions. 
%Specifically, the parameters in \texttt{VSACFG} instruction for executing 16-bit 3$\times$3 convolution computations using the FFCS strategy, are decoded by VIDU and subsequently sent to functional units. 
%The memory access instructions, \texttt{VSALD} and \texttt{VLE}, are responsible for loading $I_{0}$ and $K_0$\&$K_1$ into the VRFs, which is partitioned for inputs, weights, and accumulation data.
%}
% The \texttt{VSACFG} configuration-setting instruction is executed during the setup stage for parameters configuration, followed by the \texttt{VSALD} and \texttt{VSAM} instructions in the compute stage, as explained in Sec.~\ref{subsec: instr_design}.
% The parameters in \texttt{VSACFG} instruction, such as data precision, convolution kernel size, and dataflow strategy, are decoded by the VIDU and then sent to each scalable module.
%, as shown in Fig.~\ref{fig:dataflow_implement}.
% The customized instruction \texttt{VSALD} and official instruction \texttt{VLE} load inputs and weights of different vector lengths, i.e., $I_{0}$ and $K_0$\&$K_1$, according to the parameters received from VIDU, and store them in the VRFs.
% After the data loading is complete, the 2-stage execution of the \texttt{VSAM} instruction begins.

% \jOneFC{The 2-stage execution of the \texttt{VSAM} instruction starts when data loading is completed.}
% The processing in each stage can be divided into three steps: \ding{202}~data-requesting; \ding{203}~computing; and \ding{204}~write-back to the VRFs.

% 每条自定义算术指令可以perform多个stage的运算。具体来说，每个处理阶段都包括三个相同的基本步骤：数据加载、中间计算和结果存储。
\WX{After completion of data loading, the \texttt{VSAM} instruction initiates the execution for convolution operations, where each customized arithmetic instruction enables performing operations across multiple stages. 
%2-stage execution
Specifically, each stage comprises three fundamental steps: \ding{202}~data-requesting; \ding{203}~computing; and \ding{204}~write-back to the VRFs. 
In the \ding{202}~data-requesting step, inputs, weights, and accumulation data are requested in different priorities from VRFs and then placed into their respective queues, which serve as temporary storage for the requested data. 
During the \ding{203}~computing step, inputs I--\ding{192} are multiplied by weights W--\ding{192}. 
%Additionally, due to 
Thanks to the subsequent addition between accumulation data and computed results, the request for accumulation data and multiplication computations can be executed concurrently, effectively overlapping the data-requesting with computing steps. 
In the \ding{204}~write-back step, the data of the result queue are written back to the VRFs. 
The concurrent accessibility of the three partitions within the VRFs allows the data-requesting step of the next stage to overlap with the current stage.}


%\rFourCN{Each customized arithmetic instruction enables to perform operations across multiple stages. 
%The 2-stage execution of the \texttt{VSAM} instruction starts when data loading is completed.
%Specifically, each stage comprises three fundamental steps: \ding{202}~data-requesting; \ding{203}~computing; and \ding{204}~write-back to the VRFs.}

% In the \ding{202}~data-requesting step, the operand requester issues requests to the VRFs for inputs, weights, and accumulation data with different priorities.
% The required data are obtained based on the address information in the requests and then located into the corresponding queues.
%\rFourCN{In the \ding{202}~data-requesting step, inputs, weights and accumulation data are requested from VRFs with different priorities and then located into the corresponding queues.}
% The computing step begins when the input queue and weight queue are ready.
% \rOneCN{During the \ding{203}~computing step, the input queue and weight queue send the corresponding data I--\ding{192} and W--\ding{192} to the tensor core.}
%\rFourCN{During the \ding{203}~computing step, inputs I--\ding{192} are multiplied by weights W--\ding{192}.}
% Since the accumulation data does not participate in the MAC operations inside the PE, the request priority is lower than inputs and weights. 
% Therefore, the accumulation data can be requested during the computing step, which realizes the effective overlap of the data-requesting and computing steps and improves the computation efficiency.
% 由于accumulation data在乘法，因此accumulation data的请求 and 乘法computing可以同时进行，实现了1、2这两个step的有效overlap.
%\rFourCN{Additionally, due to the subsequent addition between accumulation data and computed results, the request for accumulation data and the multiplication computations can be executed concurrently, which realizes the effective overlap of the data-requesting and computing steps.}
%\rFourCN{In the \ding{204}~ step, the data in the result queue are written back to the VRFs.
%The concurrent accessibility of the three partitions within the VRFs enables the data-requesting step of the next stage to overlap with the current stage.}
% 由于VRFs的三个分区可以被同时访问，因此下一个stage的data-requesting step 可以与当前stage实现overlap。
% \rFourCN{The accumulation data can be requested during the computing step, which realizes the effective overlap of the data-requesting and computing steps.}
% When the addition between the results of a complete convolution computation and the requested accumulation data is finished, the partial sums of current stage are sent to the result queue.
% \rOneCN{When the accumulation between results and the requested data is finished, the partial sums of the current stage are sent to the result queue.}
% \rOneCN{In the \ding{204}~third step, the data in the result queue is written back to the VRFs at AMEM1, and the data-requesting step of the second stage starts.}
% Note that the request address for accumulation data and the write-back address in VRFs are the same, i.e., AMEM1.
% In the data-requesting step of the second stage, the input-request has different address information from the input-request of the first stage, obtaining the corresponding I--\ding{193}. 
% \rOneCN{The inputs of the second stage are I--\ding{193} due to different address information within the request, and weights are reused from the previous stage to achieve high data reuse.}
% The address information of the weight-request remains the same, thus achieving the reuse of W--\ding{192} data.
% The computing and write-back steps of the second stage are similar with the first stage except for the address of accumulation data, which is AMEM2 at VRFs.
% Under the scheduling of customized instructions, the specifically optimized dataflow strategies fully exploit the parallel processing advantages of the hardware, enhancing data utilization and computational efficiency.
% The implement saves on-chip storage space and reduces energy consumption, achieving efficient inference for various DNNs.

\WX{Thus, in collaboration with the instructions and dataflow strategy, SPEED achieves efficient parameter configuration, data scheduling, and computation in MP-DNNs inference deployment. 
In particular, the customized instructions enable a high overlap when executing multi-stage operations, and the configurable multi-precision dataflow strategy fully leverages data reuse opportunities, efficiently enhancing computational and energy efficiency.}

%\rFourCN{By coordinating the instructions and dataflow strategy, efficient parameter configuration, data scheduling, and computation are achieved. In particular, the configurable multi-precision dataflow strategy fully leverages data reuse opportunities to reduce power consumption. Moreover, the customized instructions enable a high overlap when executing multi-stage operations, which enhances computational efficiency. Consequently, the dataflow strategy coordinated with instructions effectively supports the efficient inference of MP-DNNs.}
% 通过指令集与数据流的协同工作，实现了高效的参数配置、数据调度和计算。
% 特别是，可配置的多精度数据流通过完全利用数据重用机会，显著降低了功耗。
% 此外，专用化自定义指令在执行多阶段操作时具有较高的重叠度，从而显著提升了计算效率。
% 因此，与指令协调的数据流策略有效地支持了MP-DNNs的高效推理。
% \rOneCN{
% The specific dataflow strategy fully leverages the multi-dimension parallelism provided by the hardware architecture, leading to significant improvements in computational efficiency.
% Moreover, the sufficient data reuse opportunities of dataflow strategy effectively minimize on-chip storage requirements and reduce energy consumption. 
% % Consequently, it enables efficient inference for MP-DNNs.}
% thereby realizing efficient inference for multi-precision quantized DNNs.



==> 4-res.tex <==
% \begin{table}[!htb]
% % \caption{Hardware Architecture Parameters Used in the Experiments} 
% \caption{\rThreeCN{Configurable Parameters of the SPEED Hardware Architecture}} 
% % \caption{Hardware Architecture Parameters} 
% \label{tab:archi_paras}
% \centering
% \renewcommand \arraystretch{1.25} 
% \resizebox{0.42\textwidth}{!}{
% \begin{tabular}{>{\raggedright\arraybackslash}p{0.45\linewidth}|>{\centering\arraybackslash}p{0.40\linewidth}}
% \hline
% \textbf{Parameters} & \textbf{Values}      \\ \hline
% \#Lanes                         & {[}2, 4, 8{]} \\
% \#TILE\_R / \#TILE\_C           & {[}2, 4, 8{]} \\
% VRF Size                         & 16 KiB      \\
% Vector Length                    & 4096 bit    \\ \hline
% \end{tabular}
% }
% \end{table}

\section{Experimental Results}\label{sec:res}
% The aforementioned processor designs in RTL are synthesized by Synopsys Design Compiler and implemented under SIMC 28-nm process.The Synopsys Design Compiler is used to obtain the power, performance and area (PPA) values.
% \subsection{Performance Analysis}

\subsection{Experimental Setup}\label{subsec:setup}
% To highlight the effectiveness of our design, in the following sections, we provide a detailed description of the experiments, including performance evaluations at the operator and model levels, area overhead, and we trade off area efficiency and throughput under various architecture parameters.
\jOneFC{To demonstrate the effectiveness of the proposed SPEED processor, we first evaluate the performance and area overhead of SPEED and explore the trade-offs between area efficiency and throughput under various architecture parameter configurations,}
\WX{where Ara~\cite{Cavalcante2022NewAra}, the pioneer open-source implementation of RVV processors, are chosen as the baseline design for comparison.}
%\jOneFC{Ara\cite{Cavalcante2022NewAra}, the pioneer open-source implementation of RVV processors, serves as our baseline design for comparison.}
% The varying architecture parameters are shown in Table~\ref{tab:archi_paras}. 
% For a comparison purpose, we choose Ara\cite{Cavalcante2022NewAra} as the baseline design, which is the first open-source implementation of RISC-V vector processor. 
%\jOneFC{Ara\cite{Cavalcante2022NewAra}, the pioneer open-source implementation of RVV processors, serves as our baseline design for comparison.}
% Moreover, we configure both SPEED and Ara with 4 lanes and a vector length of 4096 bits, and in order to ensure an equivalent number of MACs as Ara, we set both \#TILE\_R and \#TILE\_C of MPTU in each SPEED’s lane to 2.
\jOneFC{To ensure a fair comparison and to match the computational capacity of Ara, SPEED and Ara are both configured with 4 lanes, each having a vector length of 4096 bits. 
% Additionally, the MPTU in each lane of SPEED is configured with \#TILE\_R and \#TILE\_C parameters set to 2, aligning with Ara's MAC count.
% Additionally, the MPTU in each lane of SPEED is configured with \#TILE\_R and \#TILE\_C parameters equal to 2, establishing an equivalent number of MAC operations as in Ara's design.
Additionally, to ensure that the MPTU in each lane of SPEED performs the same number of MAC operations as Ara's design, the MPTU is configured with \#TILE\_R and \#TILE\_C parameters, both equal to 2.}
% To demonstrate the capabilities of SPEED on MP-DNN workloads, we benchmark various convolution kernels and several popular MP-DNNs, including VGG16\cite{Liu2015VGG16}, ResNet18\cite{He2016ResNet}, GoogLeNet\cite{Szegedy2015Googlenet}, MobileNetV2\cite{Sandler2018MobileNet}, ViT-Tiny\cite{Yuan2021ViT}, ViT/B-16\cite{dosovitskiy2021an}.

\jOneFC{To present SPEED's computational efficiency on MP-DNN workloads, we conduct benchmarks across a wide range of convolutional kernels and leading MP-DNN models that encompass a variety of MP-DNN operators, such as CONV, PWCV, DWCV, and MM. 
These models include VGG16\cite{Liu2015VGG16}, ResNet18\cite{He2016ResNet}, GoogLeNet\cite{Szegedy2015Googlenet}, MobileNetV2\cite{Sandler2018MobileNet}, ViT-Tiny\cite{Yuan2021ViT}, and ViT/B-16\cite{dosovitskiy2021an}, representing the diverse computational demands of contemporary MP-DNN applications.}
We employ \WX{\textit{performance (OPs/MAC/cycle)}} as the evaluated metric, indicating the number of \WX{valid} computational results produced per clock cycle.
\WX{The clock count is measured within different convolution and MM layers of DNNs by the cycle-accurate simulation with QuestaSim, following the experimental method in \cite{Cavalcante2022NewAra}.}
%The clock count is measured across \WX{the convolution and MM layers in DNNs} with the cycle-accurate simulation with QuestaSim, which follows the experimental method in \cite{Cavalcante2022NewAra}.
%across the convolutional layer and MM layer in the DNNs 
% To evaluate the impact of our architectural modifications at the hardware level, we synthesize both SPEED and Ara using Synopsys Design Compiler 2014.09 on the TSMC 28 nm process.
% Furthermore, we compare the throughput and area efficiency under different combinations of architecture parameters for \#Lanes, \#TILE\_R, and \#TILE\_C to discuss the real performance limitation of the SPEED architecture.
\jOneFC{Furthermore, we synthesize both SPEED and Ara using Synopsys Design Compiler 2014.09 on the TSMC 28 nm process to explore the design space and analyze the trade-offs between throughput and area efficiency.
The analysis provides insights into the scalability and adaptability of SPEED's architecture to different MP-DNN workloads.}
Finally, we conduct a comprehensive comparison between our design and several state-of-the-art RISC-V processors\cite{Cavalcante2022NewAra, Cavalcante2020AraA1TVLSI, Perotti2023Yun, Askarihemmat2023QuarkAI, Theo2023sparq} \WX{to demonstrate the superior performance of SPEED in MP-DNN deployments.}
%to demonstrate the advantages of SPEED in MP-DNN deployments.

% \begin{table}[!htb]
% % \caption{Hardware Architecture Parameters Used in the Experiments} 
% \caption{Hardware Architecture Parameters} 
% \label{tab:archi_paras}
% \centering
% \renewcommand \arraystretch{1.25} 
% \resizebox{0.42\textwidth}{!}{
% \begin{tabular}{>{\raggedright\arraybackslash}p{0.45\linewidth}|>{\centering\arraybackslash}p{0.40\linewidth}}
% \hline
% \textbf{Parameters} & \textbf{Values}      \\ \hline
% \#Lanes                         & {[}2, 4, 8{]} \\
% \#TILE\_R / \#TILE\_C           & {[}2, 4, 8{]} \\
% VRF Size                         & 16 KiB      \\
% Vector Length                    & 4096 bit    \\ \hline
% \end{tabular}
% }
% \end{table}

% \rTwoCN{In the following sections, we will use the word performance (OP/cycle) to indicate the number of useful computational operands per clock cycle, and we measure the cycle count of the same benchmarks of Ara\cite{Cavalcante2022NewAra} with a cycle-accurate simulation of our vector processor using Questasim.}
% \rOneFC{In the following sections, the term `performance' (OP/cycle) refers to the number of computational operations per clock cycle of a RISC-V processor.}
% \rOneFC{To evaluate the performance of SPEED, we utilize different benchmarks at both the operator and model levels. The operator-level benchmarks include various convolutional operators, while the model-level benchmarks encompass four popular DNNs.}
% \rOneFC{Note that when being evaluated using DNNs, the performance of SPEED is derived by calculating the ratio of the total number of operations to the cumulative number of inference cycles across the convolutional layers in the network.}
% \rOneFC{Note that the performance of SPEED at the model-level evaluation is measured by the ratio of total operations performed to the number of inference cycles across the convolutional layers in the DNN model.}
% The performance of DNNs in terms of speed is measured by the ratio of total operations performed to the number of inference cycles across the convolutional layers.
% \rOneFC{To ensure a fair comparison between Ara~\cite{Cavalcante2022NewAra} and SPEED, we measure the cycle count of the selected benchmarks following the experimental method in \cite{Cavalcante2022NewAra}, which employs cycle-accurate simulation with QuestaSim.}
% \rTwoCN{
% % For the whole DNN inference, our performance is derived by calculating the ratio of the total number of operands to the cumulative number of inference cycles across the convolutional layers in the network.
% For the whole DNN inference, our performance is derived by calculating the ratio of the total operands to the cumulative inference cycles across the convolutional layers in the network.}
% \rOneFC{To evaluate the impact of our architectural modifications at the hardware level, we synthesize our four-lane SPEED, and each lane in SPEED contains a SAU with both $TILE\_R$ and $TILE\_C$ parameters set to 4. The vector length is set to the same as Ara. The synthesis was performed using Synopsys Design Compiler on TSMC 28 nm process.}
% \rOneFC{Finally, we make a comprehensive comparison between SPEED and several prior state-of-the-art RISC-V processors to show the effectiveness of SPEED.}
% \rOneFC{Finally, we conduct a comprehensive comparison between SPEED and several state-of-the-art RISC-V processors \cite{Rossi2021VegaAT, Garofalo2021ESSCIRC, Garofalo2023DARKSIDEAH, Cavalcante2022NewAra, Perotti2023Yun} to show the effectiveness of SPEED in multi-precision DNN deployments.}
% \rTwoCN{SPEED's instance was configured with four lanes, and the user-defined TILE\_R and TILE\_C parameters of the SAU within each lane were set to 4.
% The processor designs in RTL are synthesized by Synopsys Design Compiler and implemented under a 28-nm process. The Synopsys Design Compiler is used to obtain the power, performance, and area (PPA) values.}

% \begin{figure}[!htbp]
% \centering  
% \subfigure
% % [ Performance scaling for FF and CF dataflow strategies, as compared to the baseline Ara.]
%     []{  
%         \begin{minipage}{0.45\linewidth}
%         \centering  
%         \includegraphics[width=\linewidth]{figures/operator_eval_input_tensor.pdf}
%         \end{minipage}
%     }
% \subfigure
% % [ Examples on kernel distributing weight parameters to SA core for the Conv3 layer]
%     []{  
%         \begin{minipage}{0.45\linewidth}
%         \centering     
%         \includegraphics[width=\linewidth]{figures/operator_eval_input_channel.pdf}
%         \end{minipage}
%     }
% \caption{Operator-level comparison of Ara and SPEED: 
% % (a) FF and CF dataflow strategies; 
% (a) Different dataflow strategies;
% (b) Multi-precision performance using a conv3x3 operator.}   
% \label{fig:FF_CF}  
% \end{figure}

% \begin{figure}[htb]
%     \centering
%     \subfloat[]{\includegraphics[width=1\linewidth]{figures/access_size.pdf}}
%     \hfill
%     \subfloat[]{\includegraphics[width=1\linewidth]{figures/input_tensor.pdf}}
%     \caption{Operator-level comparison of Ara and SPEED: 
% % (a) FF and CF dataflow strategies; 
% (a) DRAM access size between Ara and different dataflow strategies;
% (b) Performance result comparisons between Ara and different dataflow strategies under various kernel-size configurations.}
%     \label{fig:op_level}
% \end{figure}

\subsection{Operator-level Evaluation}\label{sec:opera_level}
%为了展示混合数据流的优势并通过讨论其在不同种类的内核情况下的适配性，以验证前面章节的设计目的，在本章节中，我们对各种数据流的DRAM access size以及performance进行了对比。
% Sec.~\ref{subsec: conv_dataflow}
% \rThreeCN{To demonstrate the advantages of the mixed dataflow and confirm the design movitation of Sec.~\ref{subsec: conv_dataflow},
% this section compares the DRAM access size and performance of various dataflow strategies and discusses its adaptability under different kernel-size.
% First, we select several common DNNs input tensor sizes and compare different convolution dataflow strategies with Ara under various kernel-size to illustrate the relative size of DRAM access that mainly determine the energy consumption, as shown in Fig.~\ref{fig:access_size}.}
% \jOneFC{To demonstrate the effectiveness of the mixed dataflow of SPEED, we evaluate the performance of SPEED employing the proposed multiple dataflow strategies and compare them with Ara at the operator level.
% To ensure a fair comparison, SPEED and Ara are configured to achieve equivalent peak throughput, as detailed in Sec.~\ref{subsec:setup}.}

\modimt{(To be deleted) Modified text according to IV.3}

\jOneFC{This subsection delves into the operator-level evaluation, employing various dataflow strategies on SPEED and comparing them against Ara to demonstrate the effectiveness of the proposed mixed dataflow.}
\jOneFC{To ensure a fair comparison, SPEED and Ara are configured to achieve equivalent peak throughput, as elaborated in Sec.~\ref{subsec:setup}.}
\jOneFC{We first explore the efficient data reuse during computation under different dataflow strategies, as reflected in the DRAM access size,} \WX{which is a key metric for evaluating energy and computational efficiency.}
%which is a key metric of energy consumption and computational efficiency.}
\jOneFC{In addition, performance serves as a direct measure of effective throughput on various DNN workloads.}
\jOneFC{Therefore, at the operator-level evaluation, we focus on exploring these key metrics to present the efficiency of SPEED under various DNN operators.}

% relative volume of DRAM access that mainly determine the energy consumption, as shown in Fig.~\ref{fig:op_level}~(a).
% \rThreeCN{The kernel sizes in the experiments are PWCV, CONV$3$$\times$$3$, DWCV$3$$\times$$3$ (s = 2), and CONV$5$$\times$$5$.
\jOneFC{The benchmark DNN operators are PWCV, CONV$3$$\times$$3$, DWCV$3$$\times$$3$ (s = 2), and CONV$5$$\times$$5$, which are among the most common and computation-intensive operators in DNNs.}
\rThreeCN{Here, CONV$k$$\times$$k$ refers to the standard convolution kernel with a size of $k$, and DWCV$k$$\times$$k$ indicates the depth-wise convolution kernel, also of size $k$.
Additionally, `s'  represents the stride, a parameter that defines the step length in convolution operations.}

% To show more clearly the difference between different dataflow strategies, we geometrically averaged the relative size of DRAM access for different input tensor sizes.
% It can be observed that the DRAM access size of Ara is significantly larger than that of other dataflow strategies in the case of PWCV.
% \jOneFC{As shown in Fig.~\ref{fig:access_size}, the DRAM access size of Ara is significantly larger than that of other dataflow strategies in the case of PWCV.}
% \jOneFC{Fig.~\ref{fig:access_size} illustrates how SPEED's various dataflow strategies effectively reuse data, enhancing computational efficiency and significantly reducing off-chip DRAM access.}

% \begin{figure}[!htbp]
%   \centering
%     \includegraphics[width=0.92\columnwidth]{figures/access_size.pdf}
%       % \caption{FF vs. CF and mi$\times$ strategies layer-wise performance for GoogleNet.}
%       % \caption{DRAM access size between Ara under different dataflow strategies.}
%       %\caption{\jOneFC{DRAM access size savings of SPEED that employs different dataflow strategies in comparison with Ara.}}
%       \caption{\WX{DRAM access size savings in SPEED that employs different dataflow strategies compared to Ara.}}
%         \label{fig:access_size}
% \end{figure}

\begin{figure}[!htbp]
  \centering
    \includegraphics[width=0.92\columnwidth]{figures/r1_access_size.pdf}
      % \caption{FF vs. CF and mi$\times$ strategies layer-wise performance for GoogleNet.}
      % \caption{DRAM access size between Ara under different dataflow strategies.}
      %\caption{\jOneFC{DRAM access size savings of SPEED that employs different dataflow strategies in comparison with Ara.}}
      \caption{\reFirCN{External memory access size savings in SPEED that employs different dataflow strategies compared to Ara.}}
        \label{fig:access_size}
\end{figure}

%\rFourCN{Fig.~\ref{fig:access_size} illustrates how SPEED's various dataflow strategies effectively reuse data, significantly reducing off-chip DRAM access.}
\WX{Fig.~\ref{fig:access_size} exhibits various dataflow strategies in SPEED to effectively reuse data, significantly reducing off-chip DRAM access.}
% The relative DRAM access size of FFCS, CF and FF dataflow strategies are 12.12\%, 47.12\%, 9.81\% of Ara, respectively, which indicates that Ara produces the greater energy consumption.
\jOneFC{Specifically, in the evaluation of the PWCV operator, the relative DRAM access size of SPEED using FFCS, CF, and FF dataflow strategies are merely 12.12\%, 47.12\%, and 9.81\% of Ara, respectively, leading to notable reductions in off-chip memory access and improved computational efficiency.}
% For DWCV$3$$\times$$3$ condition, the DRAM access size of FF dataflow strategy optimized for depth-wise operations is 15.92\% relative to Ara.
% 对于DWCV operator，由于FFCS和CF策略都针对input channel维度上的叠加计算做了优化，所以并不适用，因此SPEED采用FF策略。
\WX{Considering that both FFCS and CF strategies, developed for computations along the input channel dimension, are not applicable for the DWCV$3$$\times$$3$ operator, SPEED employs the FF strategy optimized for depth-wise operations, which achieves a DRAM access size significantly reduced to 15.92\% of Ara’s.}
%\jOneFC{For \WX{the} DWCV$3$$\times$$3$ operator, 
%\rFourCN{both FFCS and CF strategies, which are developed for computations along the input channel dimension, are not applicable. Therefore,}
%SPEED employs the FF strategy optimized for depth-wise operations and achieves a DRAM access size significantly reduced to 15.92\% of Ara's.}
% \rThreeCN{Under different kernel-size conditions, the relative DRAM access size of FFCS and FF dataflow strategies are 12.12\%$\sim$64.89\% and 9.81\%$\sim$29.78\%, respectively, compared to Ara.}
%  相比于Ara，在除了DWCV算子情况下，采用FFCS方法的SPEED实现了35.11%到87.88%的DRAM access size下降。同时，在所有算子情况下，采用FF数据流的SPEED相比Ara实现了70.22%到90.19%的size减少。
\rFourCN{
% Furthermore, across the evaluations of aforementioned operators, SPEED's adoption of the FF strategy realizes a DRAM access size reduction of 70.22\% to 90.19\% against Ara.
\jOneFC{Furthermore, based on the evaluation of the benchmark operators,}
\WX{SPEED employs the FF strategy for different operators to reduce DRAM access size by 70.22\% to 90.19\% against Ara.}
%SPEED employing the FF strategy significantly reduces DRAM access size by 70.22\% to 90.19\% against Ara.}
Excluding the DWCV$3$$\times$$3$ operator, SPEED utilizing the FFCS strategy achieves \WX{significant savings in} DRAM access size ranging from 35.11\% to 87.88\% compared to Ara.}

\begin{figure*}[!tbp]
  \centering
    \includegraphics[width=2\columnwidth]{figures/r1_input_tensor.pdf}
    \vspace{-10pt}
    \caption{\reFirCN{Performance comparison of SPEED that employs different dataflow strategies with Ara across various DNN operator configurations.}}
    \label{fig:perf_kernel}
    \vspace{-1em}
\end{figure*}

% \rThreeCN{The second comparison is made on the performance of different dataflow strategies under 16-bit precision condition, and the comparison results are shown in Fig.~\ref{fig:perf_kernel}.
% The results illustrate that the performance of the three dataflow strategies of the mixed dataflow strategy perform better than Ara across various kernel sizes.
% \vspace{-8pt}
\jOneFC{Fig.~\ref{fig:perf_kernel} shows the evaluation of the performance of SPEED employing dataflow strategies in contrast with Ara under 16-bit precision DNN operators.}
% \rThreeCN{The results demonstrate that the performance of the three individual dataflow strategies within the proposed mixed dataflow, surpasses that of the Ara architecture across a range of kernel sizes.}
% }
% \rFourCN{As shown in Fig.~\ref{fig:perf_kernel}, the evaluation of the performance of SPEED employing three individual dataflow strategies are conducted in contrast with Ara under 16-bit precision DNN operators.}
% Furthermore, Ara exhibits degraded performance under conditions of smaller input tensor sizes, while the DNN models have a higher proportion of layers with smaller input tensor size and more input channels.
% \rThreeCN{Furthermore, Ara exhibits degraded performance when dealing with smaller input tensor sizes, a scenario that is common in DNN models where many layers have smaller input tensors coupled with more input channels.
% Consequently, Ara struggles to achieve efficiency in the inference of complete MP-DNN workloads.}
% \rFourCN{Among the results of aforementioned operators, SPEED maintains relatively stable inference performance despite the decreasing size of the input tensor, while Ara experiences a correspondingly decline in performance.}
\jOneFC{SPEED demonstrates consistently impressive inference performance across varying input tensor sizes, outperforming Ara which experiences a significant drop in performance with smaller tensors.}
% As expected in Sec.~\ref{subsec: conv_dataflow}, the CF dataflow strategy enhances computational efficiency by reducing the data transmission delay inside the stage. 
% This advantage is particularly obvious in the execution of PWCV, leading to computational efficiency improvements of 5.21$\sim$88.56$\times$, 3.86$\sim$4.16$\times$ and 4.36$\sim$4.58$\times$ for Ara, FFCS, and FF dataflow strategy respectively.
% 在PWCV的评估中，使用CF策略的SPEED得到了很大的性能提升，在不同input tensor size条件下，与Ara相比实现了5.21$\sim$88.56$\times$的性能提升。
% \rFourCN{In the evaluation of PWCV operator, SPEED utilizes the CF strategy, significantly outperformed Ara with a 5.21$\times$ to 88.56$\times$ performance increase across various input tensor sizes.}
% \jOneFC{This advantage is particularly evident in the evaluation of the PWCV operator, where SPEED utilizing the CF dataflow strategy achieves a performance improvement of 5.21x to 88.56x compared to Ara.}
\jOneFC{In terms of the PWCV operator, SPEED, employing the CF strategy, significantly outperforms Ara with performance improvements ranging from 5.21$\times$ to 88.56$\times$ across different input tensor sizes.}
Similarly, for \WX{the} DWCV$3$$\times$$3$ operator, the performance enhancement of the SPEED with FF strategy ranges from 1.06$\times$ to 11.27$\times$ compared to Ara.
% In the case of DWCV$3$$\times$$3$, the performance enhancement of the FF dataflow strategy ranges from 1.06$\times$ to 11.27$\times$ compared to Ara.
% Under different kernel-size conditions, the performance of FFCS and FF dataflow strategies are 1.09$\sim$21.91$\times$ and 1.03$\sim$19.91$\times$ of Ara, respectively.
% \rFourCN{Under CONV$3$$\times$$3$ and CONV$5$$\times$$5$ operators, SPEED's implementation of the CF strategy exhibits performance improvements range from 1.38 to 15.29$\times$ and 1.21 to 22.94$\times$ those of Ara, respectively.}
\jOneFC{Under CONV$3$$\times$$3$ and CONV$5$$\times$$5$ operators, SPEED within the CF strategy exhibits performance improvements ranging from 1.38$\times$ to 15.29$\times$ and 1.21$\times$ to 22.94$\times$ over Ara, respectively.}

\vspace{-12.5pt}
% \rFourCN{By considering the DRAM access size and performance metrics of SPEED with the three individual different strategies as presented above, we proceed to a detailed discussion on the most appropriate strategies for various operator types.}
\jOneFC{Considering the DRAM access size and performance metrics of SPEED with the three individual strategies, we can determine the most suitable strategies for different operator types.}
\jOneFC{As shown in Fig.~\ref{fig:access_size} and Fig.~\ref{fig:perf_kernel}, there is a trade-off between DRAM access size and performance for the FFCS, CF, and FF strategies across various kernel sizes.}
\jOneFC{The CF strategy prioritizes performance compared to other proposed strategies and excels in PWCV operations due to its optimized data scheduling.
However, its high DRAM access size can increase energy consumption.}
\jOneFC{In contrast, the FFCS strategy strikes a balance between performance and memory access for CONV operators. It maintains a lower DRAM access size than Ara while achieving performance close to the CF strategy for larger kernels.}
\jOneFC{Finally, the FF strategy focuses on optimizing data reuse within the input feature map, leading to the lowest DRAM access size among all strategies, making it particularly suitable for DWCV operations where each input channel is processed independently.}
% \jOneFC{Based on the above analysis, our mixed dataflow scheduling includes CF, FFCS, and FF strategies, and dynamically adjusts according to the characteristics of different operator types to fully exploit the advantages of each strategy.}
\jOneFC{Based on the above analysis, our mixed dataflow scheduling includes CF, FFCS, and FF strategies for PWCV, CONV, and DWCV operations, respectively, which leverages the strengths of each strategy and achieves an optimal balance between performance, energy consumption, and memory access.}
% \rThreeCN{
% As depicted in Fig.~\ref{fig:access_size} and Fig.~\ref{fig:perf_kernel}, we can notice the trade-off between DRAM access size and the performance between the FFCS, CF and FF dataflow strategy under different kernel size conditions. 
% As depicted in Fig.~\ref{fig:access_size} and Fig.~\ref{fig:perf_kernel}, we observe a trade-off between DRAM access size and performance for the FFCS, CF, and FF dataflow strategies under various kernel sizes, tailored to accelerate specific kernel types. 
% 结合上文中使用三种不同strategy的SPEED在DRAM access size和性能两个方面的表现，可以推断出各个策略对应合适的operator类型。
% \rFourCN{The SPEED with the CF strategy often demonstrates superior performance compared to other strategies due to its optimized data scheduling mechanisms. 
% However, the high DRAM access size characteristic of the CF strategy can lead to increased energy consumption, making it most effective in PWCV operator, where achieving a balance between performance and energy efficiency.
% }
% The performance of the CF strategy is better than other dataflow strategies, however, its high DRAM access size leads to increased power consumption, rendering it less suitable for scenarios except for PWCV.
% For CONV, FFCS dataflow strategy demonstrates a lower DRAM access size than Ara, and when the kernel size increases, the performance of FFCS dataflow strategy approaches that of the CF dataflow strategy, hence proving it to be more suitable for above conditions.
% For CONV, the FFCS strategy maintains a lower DRAM access size compared to Ara, and its performance closely matches that of the CF strategy as kernel sizes grow, making it more appropriate for such operator.
% \rFourCN{For CONV operators, the implement of FFCS strategy in SPEED not only maintains a lower DRAM access size than Ara but also delivers performance nearly equivalent to the CF strategy, making FFCS strategy particularly well-suited for CONV operations.}
% By optimizing depth-wise operators, FF dataflow strategy has exhibited good performance in both computational efficiency and power consumption, making it well-suited for DWCV condition.
% \rFourCN{The FF strategy effectively enhances data reuse opportunity in the input feature map dimension, enabling SPEED to achieve the lowest DRAM access size and commendable performance, particularly suitable for independently processing each input channel in the DWCV operator.}
% The FF strategy leverages a high data reuse opportunity in the input feature map dimension, achieving the lowest DRAM access size and commendable performance, thus being well-suited for handling DWCV where each input channel is processed independently.
% confirms the motivation of this work.
% \rOneFC{We conduct two sets of experiments to evaluate the performance of SPEED under various precision conditions and explore the impact of different dataflow strategies. The experiments involve varying the input tensor size across several kernel sizes commonly used in DNNs.}
% \rTwoCN{
% % We designed two sets of experiments to evaluate the performance of SPEED under various precision conditions and investigate the influence of different dataflow strategies on its effectiveness.
% We design two sets of experiments to investigate the influence of different dataflow strategies on its throughput and evaluate the performance of the SPEED under various precision conditions to identify the effectiveness of the proposed contributions.}
% % We design two sets of experiments to identify the effectiveness of the proposed contributions.}
% \rOneFC{Fig.~\ref{fig:FF_CF}~(a) presents the performance of our proposed CF and FF dataflow strategies in comparison with Ara's dataflow strategy.}
% \rOneFC{Under the conv1x1 condition, the CF dataflow strategy achieves a 3.31$\times$ higher throughput compared to the FF.}
% \rOneFC{However, for kernel sizes greater than or equal to 3, the FF dataflow strategy achieves up to 2.1$\times$ higher throughput than the CF.}
% \rOneFC{Note that adopting either the FF or CF in SPEED significantly improves performance by 1.4$\times$ to 20.4$\times$ compared to Ara's dataflow strategy across all settings of convolutional operators.}
% \rOneFC{Moreover, the CF dataflow strategy exhibits a significant 3.31$\times$ higher performance than the FF for conv1x1 convolutional layers. Conversely, for convolutional layers ranging from conv3x3 to conv7x7, the FF dataflow strategy achieves up to 2.1$\times$ higher performance than the CF. Hence, the CF dataflow strategy is more suitable for small kernel convolutions, while the FF excels in handling large kernel convolutions.}
% \rOneFC{As the kernel size increases beyond 3, the FF strategy shows a substantial performance improvement, achieving up to 2.1 $\times$ higher throughput than the CF strategy.}
% \rOneFC{When the kernel size is greater than or equal to 3, the FF dataflow strategy achieves up to 2.1$\times$ throughput improvement over the CF.}
% \rTwoCN{
%讲清楚实验是如何设计出来的（两种策略在什么情况下做的）
% We evaluate the performance of various dataflow strategies by changing the input tensor size across several kernel sizes commonly employed in DNNs.
% The performance of various dataflow strategies is shown in \Rone{Fig.~\ref{fig:FF_CF} (a)}. 
% The CF strategy demonstrates a performance improvement over the FF strategy in the convolutional kernel condition of conv1x1, achieving a throughput that is 3.31 $\times$ higher. 
% As the kernel size increases, the performance of the FF strategy improves significantly, up to 2.1 $\times$ better than the CF strategy. This demonstrates the effectiveness of the FF strategy in supporting large-scale convolution operations. 
% Moreover, our work demonstrates upper performance of throughput over Ara across all convolutional kernel scenarios, particularly excelling in the conv7x7 condition with an input feature map size of 16, resulting in a 20.4 times performance improvement.
% Moreover, our work demonstrates better throughput performance compared to Ara across all convolutional kernel scenarios, particularly resulting in a 20.4 $\times$ improvement in performance under the conv7x7 condition.}
%感觉下面这句可以不要
% Therefore, combining the strengths of FF and CF strategies, adopting distinct data dataflow strategies for different convolutional layers is a more optimal approach.}
%记得讲FF在尺寸增加下 优势增长快 与此同时 两个都比Ara好
% \rOneFC{Fig.~\ref{fig:FF_CF}~(b) shows SPEED's superior and stable performance across varying input tensor sizes in multi-precision computation compared to Ara.}
% \rOneFC{When operating with 8 bits, SPEED outperforms Ara by 2.1$\times$ at least in terms of performance.}
% \rOneFC{Moreover, Ara exhibits degraded performance as the input tensor size decreases while DNNs execute deeper layers, which attributes to inefficient Ara's dataflow strategy as discussed in Sec.~\ref{subsec:mix_flow}.}
% \rOneFC{By contrast, SPEED maintains high performance across varying input tensor sizes, making it efficient for multi-precision DNN tasks.}
% \rOneFC{SPEED achieves a significant 2.1$\times$ performance improvement over Ara's optimal  of 64 OP/cycle}
% \rOneFC{}
% \rOneCN{To evaluate the performance of SPEED in multi-precision computation under various input tensor size, we conduct a comparative throughput analysis against Ara, using conv3x3 as a benchmark, as it is more commonly used in DNNs.}
%为了不同input size对性能的影响，做了什么实验 得到什么结论
% As depicted in \Rone{Fig.~\ref{fig:FF_CF} (b)}, SPEED demonstrates a better performance over Ara across 4-16 bit, 
% \rTwoCN{the input tensor size diminishes as the DNNs undergoes deeper layering, and Ara exhibits suboptimal performance with reduced input tensor sizes owing to its inherent dataflow design. Conversely, SPEED continues to demonstrate commendable proficiency in such scenarios.}
% \rTwoCN{SPEED demonstrates more robust performance across varying input tensor sizes, as depicted in \Rone{Fig.~\ref{fig:FF_CF} (b)}. 
% At the same time, due to the shortcomings in Ara's dataflow design, as discussed in Section III-D, Ara exhibits a degradation in performance as the input tensor size decreases while DNNs execute deeper layers. 
% However, Ara exhibits a degradation in performance as the input tensor size decreases while DNNs execute deeper layers, which can be attributed to the shortcomings in Ara's dataflow design, as discussed in Section III-D.
% And, especially when operating with 8 bits, SPEED outperforms Ara's optimal theoretical performance of 64 OP/cycle\cite{Askarihemmat2023QuarkAI} by a margin of 2.1$\times$.}
% Especially when operating with 8 bits, SPEED demonstrates remarkable performance, outperforming Ara's optimal theoretical processing capacity of 64 operations per cycle by a substantial margin of 2.1 times.
% This suggests that SPEED's architecture is particularly well-suited for handling multi-precision inputs, resulting in a substantial performance boost compared to Ara.}
% In this sub-section, we perform a detailed performance evaluation of the proposed vector design and its key features. 
% To demonstrate the benefits of our designs, we benchmarked SPEED and related works with various Matrix, different kernel sizes and shapes. 
% To do this, we developed customized programs for conv2d, matri$\times$ multiplication, and other common kernels needed to run typical neural networks on SPEED.
% Table~\ref{tab:MATRI$\times$ MULTIPLICATION} shows the SPEED's performance on integer MatMuls, sweeping all the main supported data formats compared with related works. 
% As anticipated, SPEED achieves performance acceleration ratios of 2.7$\times$ and 6.72$\times$ (16bit), 2.9$\times$ and 11.9$\times$ (8bit) for matri$\times$ computation at various precisions compared to the related work by Yun and Ara, primarily due to the increased parallel dimensions of data processing as well as the data utilisation of the systolic arrays.
% \begin{figure}[!tbp]
%   \centering
%     \includegraphics[width=1\columnwidth]{figures/per_model.pdf}
%       % \caption{FF vs. CF and mi$\times$ strategies layer-wise performance for GoogleNet.}
%       \caption{Comparisons of the performance between Ara and SPEED. 
%       % For the analysis, we evaluated four CNN-based and two Transformer-based benchmarks on 16-bit, 8-bit and 4-bit precisions. 
%       %SPEED provides 5.26$\times$ and 12.77$\times$ speedup over Ara at 16-bit and 8-bit precision on average, respectively.
%       \WX{On average, SPEED achieves a speedup of 5.26$\times$ and 12.77$\times$ over Ara at 16-bit and 8-bit precision, respectively.}
%       }
%         \label{fig:model_level}
% \end{figure}
\begin{figure}[!tbp]
  \centering
    \includegraphics[width=1\columnwidth]{figures/r1_per_model.pdf}
    \vspace{-10pt}
    
      % \caption{FF vs. CF and mi$\times$ strategies layer-wise performance for GoogleNet.}
      \caption{\reFirCN{Comparisons of the performance between Ara and SPEED. 
      On average, SPEED achieves a speedup of 4.88$\times$ and 11.89$\times$ over Ara at 16-bit and 8-bit precision, respectively.}
      }
    \vspace{-1em}
      
        \label{fig:model_level}
\end{figure}

\subsection{Model-level Evaluation}
% To demonstrate the performance of SPEED in MP-DNN workloads, we conduct a comprehensive performance evaluation across various popular DNNs with different precisions.
% As explained in Sec.~\ref{sec:opera_level}, we select appropriate dataflow strategies for different types of kernels within MP-DNN workloads, thereby composing the mixed dataflow strategies to ensure efficient inference.
\jOneFC{We conduct a model-level evaluation to present the performance benefits of SPEED that arise from the co-optimization of customized instructions, hardware architecture, and mixed dataflow strategies.}
\jOneFC{Four CNN-based and two Transformer-based DNN benchmarks, embracing VGG16, ResNet18, GoogLeNet, MobileNetV2, ViT-Tiny, and ViT/B-16, are evaluated under 16-bit, 8-bit and 4-bit precisions.}
% \jOneFC{SPEED demonstrates significant performance improvements over Ara across various DNN models and precision levels.}
\jOneFC{As shown in Fig.~\ref{fig:model_level}, SPEED achieves a 5.26$\times$ and 12.77$\times$ speedup over Ara on average at 16-bit and 8-bit precision, respectively.}
% On average, SPEED provides 5.26$\times$ and 12.77$\times$ speedup over Ara at 16-bit and 8-bit precision, respectively, as shown in Fig.~\ref{fig:model_level}.

% In the CNN-based benchmark evaluations, SPEED demonstrates relatively stable inference performance across various networks. 
% SPEED shows a performance improvement of 1.94$\times$ at 16-bit precision in the VGG16 model, which contains a high proportion of CONV$3$$\times$$3$ layers.
%\jOneFC{For CNN-based models like VGG16, which heavily utilize CONV$3$$\times$$3$  layers, SPEED achieves a 1.94$\times$ speedup over Ara at 16-bit precision.}
\rFourCN{For CNN-based models like VGG16, which heavily \WX{rely on} CONV$3$$\times$$3$ layers, SPEED achieves a 1.94$\times$ speedup over Ara at 16-bit precision, with advantages gained from the FFCS strategy.}
% Conversely, in ResNet18, GoogLeNet, and MobileNetV2 model, where PWCV and DWCV layers predominate, SPEED achieves performance speedup ranging from 6.63$\times$ to 71.32$\times$ at 16-bit precision and from 17.85$\times$ to 245.15$\times$ at 8-bit precision.
% \rFourCN{
% Moreover, in ResNet18, GoogLeNet, and MobileNetV2 models, where PWCV and DWCV layers are predominant, SPEED leverages the CF and FF strategies, optimized for these operators, to achieve a performance speedup of 6.63$\times$ to 71.32$\times$ at 16-bit precision and 17.85$\times$ to 245.15$\times$ at 8-bit precision, demonstrating a significant improvement.}
\jOneFC{Moreover, \WX{for} models dominated by PWCV and DWCV layers, such as ResNet18, GoogLeNet, and MobileNetV2, SPEED leverages its optimized CF and FF strategies to achieve significant speedups ranging from 6.63$\times$ to 71.32$\times$ at 16-bit precision and 17.85$\times$ to 245.15$\times$ at 8-bit precision, respectively.}
\jOneFC{For Transformer-based models like ViT-Tiny and ViT/B-16, SPEED \WX{employs a matrix multiplication dataflow strategy to deliver} a performance boost of 1.18$\times$ to 1.46$\times$ at 16-bit precision and 2.00$\times$ to 2.13$\times$ at 8-bit precision, respectively.}
% In the evaluations of ViT-Tiny and ViT/B-16 models, SPEED attains performance speedup of 1.18$\sim$1.46$\times$ and 2.00$\sim$2.13$\times$ for 16-bit and 8-bit precision, respectively. 
% These results demonstrate the advantages of matrix dataflow strategy.
% 这些结果展示出了instr, arch 和 dataflow 的联合优化带来的性能优势。
%derived from
\rFourCN{These results highlight the performance benefits \WX{from} the joint optimization of customized instructions, hardware architecture, and mixed dataflow strategies.}
In addition, SPEED enables efficient 4-bit inference with an average performance of up to 90.75 OPs/MAC/cycle, surpassing the best of Ara by 23.69$\times$ on these DNN benchmarks.
% SPEED在8-bit和4-bit时的性能表现分别是16-bit的2.98倍和5.54倍，简要分析。
% \rFourCN{SPEED's performance at 8-bit and 4-bit precision is 2.98$\times$ and 5.54$\times$ that of 16-bit precision, respectively. 
% The ideal performance gains of 4$\times$ and 16$\times$ are not fully achieved due to limitations in off-chip bandwidth, which result in increased data transfer latency and reduced processing throughput.
% }
\jOneFC{Notably, SPEED's performance at 8-bit and 4-bit precision is 2.98$\times$ and 5.54$\times$ that of 16-bit precision, respectively. 
% While not reaching the theoretical maximum gains due to off-chip bandwidth limitations, these experimental results elaborate SPEED enabling efficient low-precision inference.
}
% \rOneFC{A layer-by-layer performance evaluation of GoogLeNet is conducted on SPEED under the 16-bit condition to discuss the advantages of the mixed dataflow strategy.}
% \rOneFC{As shown in Fig.~\ref{fig:googlenet}, the mixed dataflow strategy achieves a performance improvement of 1.88$\times$ and 1.38$\times$ in comparison with the FF-only and CF-only dataflow strategies, respectively.}
% \rOneFC{Therefore, employing the mixed dataflow strategy can significantly enhance SPEED's performance for DNN deployment.}
% Based on the aforementioned conclusions, since that the GoogleNet contains various convolution types, we designed experiments to deploy GoogleNet on SPEED. 
% The performance of GoogleNet, analyzed layer by layer within different blocks, is illustrated in \Rone{Fig.~\ref{fig:googlenet}}. These findings provide evidence to support the superiority of the mi$\times$ strategy over the individual FF and CF strategies.
% \rTwoCN{To demonstrate the general applicability of SPEED in deploying a substantial multitude of DNNs, }
% \rTwoCN{To demonstrate the high performance of SPEED across different types of DNN implementations, we conduct a layer-by-layer performance evaluation of SPEED.}
%We evaluate SPEED's high performance across different DNN implementations through a layer-by-layer analysis.
% \rTwoCN{Detailed implementations of GoogLeNet are taken as examples to discuss the advantages of the mixed dataflow strategy.
% Meanwhile, the performance of the layer-by-layer implementation, which utilizes the mixed dataflow strategy, as shown in \Rone{Fig.~\ref{fig:googlenet}}.}
%逐层是怎么来的
% Upon analyzing the average performance comparison, we observe that SPEED's mixed dataflow strategy achieves a throughput improvement of 1.88$\times$ compared to the individual FF strategy and 1.38$\times$ compared to the CF strategy.
% 实验设计方式放到前面
% Specifically, we choose GoogLeNet as our benchmark due to its intricate architecture and extensive collection of convolutional layers, as depicted in \Rone{Fig.~\ref{fig:googlenet}}.
%
% \rOneCN{
% Upon analyzing the average performance comparison, it becomes evident that the mixed dataflow design strategy yields significant improvements, surpassing the individual FF and CF strategies by 1.88$\times$ and 1.38x, respectively.}
%补一下实验目的：在很多DNN上表现都很好
%这里要改一下
% \rOneFC{Furthermore, we conduct a comprehensive performance evaluation of SPEED with the mixed dataflow strategy using multiple popular DNNs, embracing VGG16, ResNet18, GoogLeNet, and SqueezeNet, across various precisions.}
% \rOneFC{As illustrated in Fig.~\ref{fig:per_model}, SPEED achieves 6.8$\times$ and 15.7$\times$ higher performance over Ara on average under 16-bit and 8-bit precision conditions, respectively.}
% \rTwoCN{Moreover, SPEED enables efficient 4-bit inference with an average performance of up to 208.1 OP/cycle, surpassing the best of Ara by 31.5$\times$ on these DNN benchmarks.}
% \rTwoCN{We also present a comprehensive performance analysis of various precisions applied to popular DNNs with mixed dataflow strategy, including VGG16, ResNet18, GoogLeNet, and SqueezeNet, as depicted in \Rone{Fig.~\ref{fig:per_model}}. 
% By geometrically averaging the performance outcomes across multiple DNN deployments, we conducted a comparative analysis of SPEED and Ara's performance under different precisions.
% By geometrically averaging the performance outcomes across multiple DNN deployments, the result show a performance improvements achieved by SPEED over Ara, particularly the 6.8$\times$ and 15.7$\times$ enhancements in 16-bit and 8-bit precision, respectively.}
% 讲清楚用的是mix-strategy
% \rOneCN{
% We present a comprehensive performance analysis of various precisions applied to popular DNNs, including VGG16, ResNet18, GoogLeNet and SqueezeNet, as depicted in \Rone{Fig.~\ref{fig:per_model}}.
% Additionally, contrasting their performance with Ara's when utilizing these networks. By geometrically averaging the performance outcomes across multiple network deployments, we find that SPEED outperforms Ara a remarkable improvement of 6.8$\times$ (16-bit) and 15.7$\times$ (8-bit), respectively.
% }
% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/area_pie.pdf}
%         \caption{\rTwoFC{Area breakdown of (a) SPEED and (b) a single lane. MPTU occupies only 12\% of the area in a single lane while achieving significant performance.}}
%     \label{fig:area_breakdown}
%     % \vspace{-1em}
% \end{figure}
\begin{figure}[!tp]
    \centering
    \includegraphics[width=1\columnwidth]{figures/r1_area_pie.pdf}
        \caption{\reFirCN{Area breakdown of (a) SPEED and (b) a single lane. MPTU occupies only 12\% of the area in a single lane while achieving significant performance.}}
    \label{fig:area_breakdown}
    % \vspace{-1em}
\end{figure}

\subsection{Area Breakdown}
\jOneFC{On top of the model-level and operator-level evaluations, we further provide a detailed analysis of the area breakdown of SPEED, providing insights into the key components contributing to the overall area.}
% \jOneFC{Fig.~\ref{fig:area_breakdown}~(a) presents the area breakdown of SPEED, which occupies a total area of 0.72 $mm^2$.}
\jOneFC{Fig.~\ref{fig:area_breakdown}~(a) shows the area breakdown of SPEED.}
% Fig.~\ref{fig:area_breakdown}~(a) illustrates the area breakdown of SPEED with a total area of 0.72 $mm^2$ to provide insights into the key components contributing to the overall area.
The majority of SPEED's area, up to 80\%, is occupied by the lanes, which are responsible for executing the core computations with the specialized MPTU.
The remaining 20\% is allocated to other components of the processor.

\jOneFC{A closer look at the lane's area allocation, as depicted in Fig.~\ref{fig:area_breakdown}~(b), reveals that the area of a lane is primarily consumed by four components: VRFs (30\%), OP Queues (24\%), OP Requester (16\%), ALU (13\%)  and MPTU (12\%).}
% \rTwoCN{Fig.~\ref{fig:area_breakdown} illustrates the area breakdown of SPEED with a total area of 1.09 $mm^2$. In this breakdown, we observed that the processor's area is predominantly occupied by the lanes, which accounts for approximately 87\% of the total area. The remaining 13\% is allocated to other components.
% The analysis of the experimental results shows that the area of the lanes is mainly occupied by three components: the OP Queues (25\%), the OP Requester (27\%), and the SAU (26\%). 
% This finding indicates that despite occupying approximately 26\% of the lane area, which is an acceptable area overhead in view of the performance improvement of the SAU.
% This result indicates that despite the use of approximately 26\% of the lane area, considering the performance improvement is mainly brought by the optimization in SAU, making it an acceptable area overhead.
%用于数据存储功能的部件占据了lane的半数以上面积，而计算模块ALU和MPTU只占了25%的面积。
Over half the area is dedicated to data storage components like VRFs and OP Queues, \WX{whereas} computing units such as the ALU and MPTU only occupy 25\% of the area.
% Notably, MPTU serves as a key component of SPEED, enabling a 23.69$\times$ performance improvement in DNN inference performance on SPEED compared to Ara. 
% Despite the substantial performance boost, MPTU accounts for only 12\% of the lane area in SPEED, which corresponds to about 2.4\% of the total area of the processor.
% And the customized unit MPTU occupies a smaller area than the vector unit ALU, demonstrating the advantage of the MPTU in terms of hardware resource consumption.
\jOneFC{Remarkably, the MPTU, occupying only 12\% of the lane area \WX{equivalent to 2.4\% of the total area}, delivers a significant 23.69$\times$ performance improvement. 
This customized MPTU even consumes less area than the vector unit ALU, highlighting its area efficiency.}
%occupying only 12\% of the lane area, which is equivalent to 2.4\% of total area,
%与此同时，MPTU这个定制化模块在面积上的占比是小于向量计算单元ALU的，展现了MPTU的设计在硬件资源消耗上的优势。

% \rOneCN{
% \Rone{Fig.~\ref{fig:area_breakdown}} shows the area breakdown of SPEED with four lanes. SPEED’s total area is 1.09 $mm^2$, the area of the processor
% is dominated by the lanes, while other amount to similarly 13\%. 
% The area of the lanes is dominated by the OP Queues (25\%), the OP Requester (27\%), and the SAU (26\%).
% The area of SAU covers approximately 26\% of the lane, which is an acceptable area overhead in view of the performance improvement of the SAU.
% }

% \begin{figure}[htb]
%     \centering
%     \subfloat[]{\includegraphics[width=1\linewidth]{figures/multi_lanes_throughput.pdf}}
%     \hfill
%     \subfloat[]{\includegraphics[width=1\linewidth]{figures/multi_lanes_ae.pdf}}
%     \caption{Design space exploration of various architecture parameters.
% % (a) FF and CF dataflow strategies; 
% (a) Throughput comparison by varying the MPTU PE array size and the number of lanes;
% (b) Area Efficiency comparison under different architecture parameters.}
%     \label{fig:multi_lanes}
% \end{figure}
% \begin{figure}[!htbp]
%   \centering
%     \includegraphics[width=1\columnwidth]{figures/multi_lanes_ae_tp.pdf}
%       \caption{Comparisons of the area efficiency between Ara and the proposed SPEED.}
%         \label{fig:multi_lanes} 
% \end{figure}

\begin{table}[!htb]
% \caption{Hardware Architecture Parameters Used in the Experiments} 
\caption{\rThreeCN{Configurable Parameters of SPEED Architecture}} 
% \caption{Hardware Architecture Parameters} 
\label{tab:archi_paras}
\centering
\renewcommand \arraystretch{1.25} 
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{>{\raggedright\arraybackslash}p{0.45\linewidth}|>{\centering\arraybackslash}p{0.40\linewidth}}
\hline
\textbf{Parameters} & \textbf{Values}      \\ \hline
\#Lanes                         & {[}2, 4, 8{]} \\
\#TILE\_R / \#TILE\_C           & {[}2, 4, 8{]} \\
VRF Size                         & 16 KiB      \\
Vector Length                    & 4096 bit    \\ \hline
\end{tabular}
}
\end{table}

% \subsection{Scalable Exploration of SPEED Architecture}\label{sec:design_space}
\subsection{Design Space Exploration of Scalable SPEED}\label{sec:design_space}

% 为了展示可扩展向量处理器在不同应用场景中的适用性，我们对SPEED和Ara在处理MP-DNNs的常用层时的面积效率和吞吐量进行了比较分析。我们选择了一系列的参数配置进行测试，这些配置的详细信息在图1中展示。通过这些实验，我们能够评估不同设计选择对性能和资源使用的影响，从而为特定应用场景提供最优的设计指导。
% To demonstrate the advantages of SPEED architecture, we measure the throughput and area efficiency by varying different parameters as presented in Table~\ref{tab:archi_paras} under the common-used layer of MP-DNNs, and compare the same measurement under different configurations of Ara.
% \rFourCN{
% To demonstrate the versatility of scalable vector processors across diverse application scenarios, we conducted a comparative analysis focusing on area efficiency and throughput for SPEED and Ara when processing common layers within MP-DNNs. 
% We systematically test a variety of parameter configurations, the details of which are provided in Table~\ref{tab:archi_paras}. 
% These experiments provided valuable insights into how different architectural configurations affect performance and resource consumption, thereby equipping us with the knowledge to tailor designs to best serve specific application requirements.
% }
% \jOneFC{We conduct a comparative analysis of area efficiency and throughput for SPEED and Ara when processing common layers of MP-DNNs.}
\jOneFC{Exploring the design space of SPEED is crucial for understanding its performance across diverse application scenarios and guiding optimal design choices for specific use cases.}
\jOneFC{We focus on two key metrics: area efficiency and throughput, which directly impact manufacturing cost and inference performance.}
\jOneFC{By delving into SPEED's design space, we can better grasp its strengths and limitations, providing valuable insights for system design and optimization.}
% \jOneFC{Therefore, a thorough exploration of SPEED's design space enables us to better understand its strengths and limitations, offering valuable guidance for system design and optimization.}
% To verify the scalability of the proposed architecture, we realize the various hardware configuration of SPEED architecture by changing the parameters as presented in Table~\ref{tab:archi_paras}, i.e. the number of the scalable modules (\#Lanes) and the MPTU PE array size (\#TILE\_R $\times$ \#TILE\_C).
% SPEED和Ara同样允许三种可拓展模块数量的配置，另外SPEED还允许九种不同的MPTU size的配置选项。
% The SPEED architecture allows three value types of \#Lanes (2\_lanes, 4\_lanes and 8\_lanes, where 2\_lanes represents \#Lanes = 2 condition), and nine different MPTU PE array size combinations (\#TILE\_R $\times$ \#TILE\_C).
% \rFourCN{Both SPEED and Ara allows configurations for three different numbers of scalable modules (2\_lanes, 4\_lanes and 8\_lanes, where 2\_lanes represents \#Lanes = 2 condition), with SPEED further enhancing its flexibility by offering nine distinct MPTU size configuration options (\#TILE\_R $\times$ \#TILE\_C).}

\jOneFC{As presented in Table~\ref{tab:archi_paras}, both SPEED and Ara support three scalable module configurations, i.e., 2\_lanes, 4\_lanes, and 8\_lanes, where 2\_lanes represents the \#Lanes = 2 condition. SPEED further offers nine distinct MPTU size configuration options, with diverse configurations of \#TILE\_R$\times$\#TILE\_C that enlarge the scalable design space.}
% We measured the throughput and area efficiency of each hardware configuration under a fixed convolution computation, the results are depicted in Fig.~\ref{fig:multi_lanes}.
% The cases of different \#Lanes are distinguished by different color, 
% and in order to provide a more clearly representation of the impact of MPTU PE array size on area efficiency, 2\_lanes and 8\_lanes are depicted with solid blue and dashed green lines, respectively, in Fig.~\ref{fig:multi_lanes} (b).
% 如图中所示，我们对比了SPEED和Ara在面积效率和吞吐量这两个关键性能指标上的表现。特别地，我们关注对成本和功耗有着显著直接影响的面积效率这一指标。

% \rFourCN{Fig.~\ref{fig:multi_lanes} presents a comparative analysis of SPEED and Ara in terms of area efficiency and throughput, with a particular focus on area efficiency, an indicator that directly impacts cost and power consumption, thereby informing our detailed evaluation and comparison of the two processors.}
% Fig.~\ref{fig:multi_lanes} illustrates the comparison between the SPEED and the Ara. 
%  得益于架构设计上的的优势，SPEED能够提供多样化的吞吐量选项，满足不同应用场景的需求。SPEED展现出显著的吞吐量优势，其吞吐量可达Ara的最高吞吐量的1.24倍到23.43倍。
% \rFourCN{Leveraging its architectural advantages, SPEED offers a versatile array of throughput options tailored to various application scenarios. 
% SPEED's throughput ranges from 1.24 to 23.43$\times$ that of Ara's highest throughput, demonstrating significant performance benefits.}
% SPEED processor can not only provide higher throughput, but also provide a wider range of throughput options. 
% \rFourCN{In addition, the area efficiency of the SPEED surpasses that of the Ara by 1.02$\sim$2.70$\times$, which proves the advantages of the joint optimization.}
%\jOneFC{As presented in Fig.~\ref{fig:multi_lanes}, SPEED, benefited from its architectural advantages, provides a wide range of throughput options tailored to different application scenarios, achieving 1.24$\times$ to 23.43$\times$ throughput improvement than Ara at 16-bit.}
\WX{Benefiting from its architectural advantages, SPEED provides a wide range of throughput options tailored to different application scenarios, achieving 1.24$\times$ to 23.43$\times$ throughput improvement than Ara at 16-bit precision, as exhibited in Fig.~\ref{fig:multi_lanes}.}
\jOneFC{Meanwhile, SPEED achieves 1.02$\times$ to 2.70$\times$ higher area efficiency than Ara, demonstrating the benefits of joint optimization among customized instructions, hardware architecture, and dataflow mapping.}
% By demonstrating the performance of different architectural configurations of SPEED in terms of throughput and area efficiency, we can discuss the area limitation of the architecture.
% 在图1中可以观察到，可拓展模块的数量对于peak吞吐量以及吞吐量的范围有着线性的影响，然而，较多的可拓展模块引入的面积消耗会导致其在相同吞吐量条件下表现出较差的面积效率。
% \rFourCN{As shown in Fig.~\ref{fig:multi_lanes}, the number of scalable modules has a linear impact on both the peak throughput and the range of achievable throughputs. 
% However, incorporating a larger number of scalable modules introduces increased area overhead, resulting in reduced area efficiency at comparable throughput conditions.}
\WX{Moreover, as the number of scalable modules in SPEED increases, it has a linear improvement in throughput with additional area overhead, which impacts the overall area efficiency.
As shown in Fig.~\ref{fig:multi_lanes}, the configuration in SPEED that achieves the peak area efficiency is the 4\_lanes, which efficiently balances processing throughput and area utilization.}
%\jOneFC{Moreover, the number of scalable modules in SPEED has a linear impact on throughput but also increases area overhead, which can reduce area efficiency. 
% The 4\_lanes configuration of SPEED achieves optimal area efficiency, striking a balance between throughput and area efficiency.
%SPEED attains its peak area efficiency with a 4\_lanes configuration, balancing processing throughput and area utilization.}
% In Fig.~\ref{fig:multi_lanes}, it can be observed that as the number of scalable modules increases, both the peak throughput and the range of throughput variation also increase.
% At the same throughput, a smaller number of scalable modules leads to higher area efficiency. 
% This is attributed to the area overhead associated with the increased control logic required for managing a larger number of scalable modules.
% \rFourCN{The SPEED processor attains its peak area efficiency with a configuration of 4\_lanes, effectively realizing the optimal balance between processing throughput and area utilization.}

% Several observations can be made from the experiment of throughput. 
% In general terms, an increase in MPTU PE array size tends to result in improved throughput. 
% However, in the case of `4$\times$8' and `8$\times$8' under 8\_lanes, the throughput is lower than that of `4$\times$4' and `8$\times$4'. 
% This decrease is attributed to the growth of \#TILE\_C, which leads to extract loading latency, discouraging effective overlap with computation time.
% Furthermore, under the same number of MPTU PEs, variations in throughput are observed for different MPTU PE array sizes,
% such as, `2$\times$8', `4$\times$4', `8$\times$2', the throughput is better when the value of \#TILE\_R is larger. 
% This trend emerges from the effective data reuse on the feature map dimension.

% In Fig.~\ref{fig:multi_lanes} (b), we could observe that the area efficiency of 4\_lanes is generally superior to that of 2\_lanes and 8\_lanes. 
% Consequently, increasing the number of scalable modules to enhance throughput can cause excessive hardware consumption.
% Moreover, under the same \#TILE\_R conditions, higher area efficiency is achieved when \#TILE\_C = 4. 
% Furthermore, under identical \#TILE\_C conditions, expanding \#TILE\_R leads to improved area efficiency, indicating that enhancing parallelism on the feature map dimension greater gains in area efficiency compared to increasing parallelism on the output channel dimension.

\begin{table*}[!htbp]
\centering
% \caption{ COMPARISON WITH THE STATE-OF-THE-ART } 
\caption{ Comparison with the State-of-the-art RISC-V Processors } 
\renewcommand \arraystretch{1.4} 
\label{tab:Related_Work_Summary}
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{cccccc}
\hline
&Ara\cite{Cavalcante2022NewAra} 
&Yun\cite{Perotti2023Yun} 
&Quark\cite{Askarihemmat2023QuarkAI}           
&Sparq\cite{Theo2023sparq}                                                                
& SPEED (Ours)$^\dagger$                    \\ \hline
Frequency 
& 500 MHz @ 0.9 V 
& \rOneCN{280 MHz @ 1.2 V}
& 1   GHz @ - V  
& 1   GHz @ 0.8 V    
& 500 MHz @ 0.9 V         \\
Technology  
& 28 nm 
& 65 nm 
& 22 nm   
& 22 nm 
& 28 nm  \\
% Architecture
% & RISC-V + Vector
% & RISC-V + Vector
% & RISC-V + Hwacha
% & RISC-V + Vector
% & RISC-V + Vector/Tensor
% \\
Chip Area ($mm^2$)  
& 0.60  
& 6.00  
& 1.09              
& 0.42                   
& 1.60                                  \\
Int. Formats (bit)         
& 8, 16, 32, and 64   
& 8, 16, 32, and 64  
& 1, 2, and 8   
& 1, 2, 3, 4, and 16    
& 4, 8, 16, 32, and 64   \\ 
Power (mW) 
& 61.14 
& -
& 97.00
& 65.60
& 274.38  \\
\hline
\multirow{3}{*}{\shortstack{Peak Int. \\ Throughput \\ (GOPS)}} 
& 10.22  (16b) 
& 12.42  (16b)     
& -   
& 20.00  (16b)            
& 62.12  (16b)             \\

& 22.90 (8b)   
& 22.95  (8b)  
& 56.00  (8b)    
& -            
& 162.98  (8b)             \\

& -            
& -
& -                  
& 30.00  (4b)        
& 350.51  (4b)            \\ \hline
\multirow{3}{*}{\shortstack{Peak Int. \\ Area Efficiency$^{\ast}$ \\ (GOPS/$mm^2$)}}  
& 17.03 (16b)
& 25.89  (16b)      
& -   
& 23.09  (16b)     
& 38.29 (16b)                         \\

& 38.25  (8b)     
& 47.74  (8b)     
& 24.92  (8b)  
& -     
& 100.46  (8b)                         \\

& -         
& -   
& -                   
& 34.64  (4b)                             
& 216.05  (4b)                  \\ \hline
\multirow{3}{*}{\shortstack{Peak Int. \\ Energy Efficiency$^{\ast}$ \\ (GOPS/W)}}  

& 167.15  (16b)
& 51.25    (16b)     
& -   
& 239.54 (16b)     
& 226.40  (16b)                         \\

& 375.36  (8b)     
& 100.50  (8b)     
& 453.60  (8b)   
& -     
& 593.99  (8b)                         \\
& -    
& -        
& - 
& 359.32  (4b)                               
& 1,277.46 (4b)                  \\ \hline
\end{tabular}
}
\begin{tablenotes}
    \item[]\scriptsize $\ast$ The metrics are calculated based on scaling rule used in \cite{EIE2016ISCAHan} under the 28nm technology, and the other indicators are reported from related papers.
    \item[]\scriptsize $\dagger$ We configure SPEED with four lanes, and \#TILE\_R and \#TILE\_C parameters are set to 8 and 4, respectively.
%     \item[]\scriptsize $\dagger$
%     A 512$\times$28$\times$28 conv3x3 multiplication on the specific processor with four lanes.
\end{tablenotes}
\end{table*}

\begin{figure}[!htbp]
  \centering
    \includegraphics[width=\columnwidth]{figures/r1_multi_lanes_ae_tp.pdf}
      % \caption{Comparisons of the area efficiency between Ara and the proposed SPEED.}
      \caption{\reFirCN{Throughput and area efficiency comparison of SPEED with varying configurations.}}
        \label{fig:multi_lanes} 
\end{figure}


% \subsection{Comparison between SPEED and the State-of-the-arts}
\subsection{Comparisons with the State-of-the-Arts}\label{sec:related_works}
% \rOneCN{
% \Rone{Table~\ref{tab:Related_Work_Summary}} makes a comprehensive comparison between SPEED and the prior state-of-the-art RISC-V processors.}
% \rOneFC{Table~\ref{tab:Related_Work_Summary} makes a comprehensive comparison between SPEED and several state-of-the-art RISC-V processors.}
% Vega\cite{Rossi2021VegaAT} is a cluster-based architecture designed for vector processing, which is implemented in 22-nm technology. 
% Darkside\cite{Garofalo2023DARKSIDEAH} and Dustin\cite{Garofalo2021ESSCIRC} also target data-parallel workloads and employ Integer Process Unit (IPU) configurations, implemented at 65 nm using tightly coupled scalar processor clusters with independent instruction fetch pipelines. 
% Vega\cite{Rossi2021VegaAT}, Dustin\cite{Garofalo2021ESSCIRC} and Darkside\cite{Garofalo2023DARKSIDEAH} target data-parallel workloads, using tightly coupled scalar processor clusters with independent instruction control and fetch pipelines, supporting low-bitwidth mixed-precision arithmetic for energy-efficient execution of DNNs. 
% Yun\cite{Perotti2023Yun} and Ara\cite{Cavalcante2022NewAra} are vector processor architectures that, like this work, employ scalable parallel computing modules with standard RVV instruction set for efficient multi-precision DNN inference. 
% Ara~\cite{Cavalcante2022NewAra}, Yun~\cite{Perotti2023Yun}, Quark~\cite{Askarihemmat2023QuarkAI}, Sparq~\cite{Theo2023sparq} are RISC-V processors designed for DNN workloads.
\jOneFC{We compare SPEED with the state-of-the-art RISC-V processors designed for DNN workloads, including Ara\cite{Cavalcante2022NewAra}, Yun\cite{Perotti2023Yun}, Quark\cite{Askarihemmat2023QuarkAI}, and Sparq\cite{Theo2023sparq}. Table~\ref{tab:Related_Work_Summary} provides a comprehensive overview of these comparisons, focusing on projected area efficiency and energy efficiency under the same 28nm process node.}
% Ara\cite{Cavalcante2022NewAra} and Yun\cite{Perotti2023Yun} are the first open-source processor and system-on-chip (SoC), respectively, implemented based on the official RVV extension ISA.
% Ara achieves an exceptional throughput improvement of up to 380× in comparison to a scalar core~\cite{zaruba2019cost}, rendering it highly efficient for tasks such as DNN inference.  
% Yun demonstrates an efficient micro-architecture that achieves the FPU utilization of about 90\% on matrix multiplication computations even for relatively small matrix sizes~\cite{Perotti2023Yun}.
% However, they lack support for low-precision data operations in quantized DNNs inference.
\jOneFC{Ara~\cite{Cavalcante2022NewAra} and Yun~\cite{Perotti2023Yun}, leveraging the official RVV extension ISA, have demonstrated high efficiency in DNN inference, with Ara achieving up to 380× throughput improvement over scalar cores~\cite{zaruba2019cost} and Yun attaining about 90\% FPU utilization in matrix multiplications\cite{Perotti2023Yun}. However, both lack native support for low-precision data operations crucial for quantized MP-DNNs.}
% Notably, Quark~\cite{Askarihemmat2023QuarkAI} supports the inference of quantized MP-DNNs by adding customized instructions to accelerate low-precision serial operations.
% Furthermore, Sparq~\cite{Theo2023sparq} enhances support for low-precision computation by introducing customized instructions, improving the performance of ultra-low-precision (e.g. 1-bit or 2-bit) computations through vectorized multiply-shift-accumulate operations.
\jOneFC{Quark~\cite{Askarihemmat2023QuarkAI} and Sparq~\cite{Theo2023sparq} address this gap by introducing customized instructions for low-precision computation, enhancing performance in ultra-low-precision (e.g. 1-bit or 2-bit) operations through vectorized techniques. 
SPEED extends this capability by supporting a broader range of data precisions and integrating high-throughput MPTU in vector lanes, enabling efficient inference for emerging MP-DNN models.
}
% \rOneCN{
% Compared to Vega\cite{Rossi2021VegaAT}, Ara\cite{Cavalcante2022NewAra} and Yun\cite{Perotti2023Yun}, SPEED can can support also mixed and lower-precision (than 8-bit) integer workloads thanks to the enhanced customized instruction set, enabling the computation of emerging DNN models. 
% Compared to Darkside\cite{Garofalo2023DARKSIDEAH} and Dustin\cite{Garofalo2021ESSCIRC}, SPEED ensures a considerable performance gain of up to 5.7×(4-bit).
% Relative to the aforementioned works, SPEED achieves the highest possible frequency and occupies the least possible area, while achieving performance improvements of at least until 2.09$\times$ (8-bit) and 5.3$\times$ (4-bit).
% }
% \rTwoCN{

% 由于上述工作与SPEED使用的是不同的工艺节点，为了进行公平的比较，其他工作也在相同的28nm工艺下进行投影，这种投影（project）基于[cite]中的缩放规则：对频率进行线性缩放，面积进行二次缩放。
% As discussed in Sec.~\ref{sec:design_space}, we choose MPTU PE array size is `8$\times$4' under 4\_lanes condition to compare with other processors due to its superior area efficiency.
% Due to the different technology nodes adopted in these works, all designs are projected under the same 28nm process for a fair comparison. 
% % This projection is based on the scaling rule used in \cite{EIE2016ISCAHan} incl linear frequency scaling, and quadratic area scaling. 
% Additionally, the metrics for comparison are the projected area efficiency and the projected energy efficiency, as shown in Table~\ref{tab:Related_Work_Summary}.

% When compared to Ara~\cite{Cavalcante2022NewAra} and Yun~\cite{Perotti2023Yun}, 
% % SPEED shows significant performance improvement for multi-precision DNN inference along with extended support for a wider range of data precision. 
% %SPEED 在8bit条件下达到了8.79倍的性能提升。
% SPEED shows 5.00$\sim$6.07$\times$ and 7.10$\sim$7.11$\times$ throughput improvement under 16-bit and 8-bit precision, respectively.
% In terms of area efficiency, SPEED achieves a 1.47$\sim$2.24$\times$ and 2.10$\sim$2.62$\times$ enhancement compared to Ara and Yun at 16-bit and 8-bit precision, respectively, and within the context of energy efficiency, SPEED has an improvement by 1.35$\sim$4.41$\times$ and 1.58$\sim$5.91$\times$, respectively.
\jOneFC{\WX{Compared} to Ara and Yun, SPEED shows significant throughput improvements, with 5.00$\sim$6.07$\times$ and 7.10$\sim$7.11$\times$ enhancements under 16-bit and 8-bit precision conditions, respectively. 
In terms of area efficiency, SPEED realizes a 1.47$\sim$2.24$\times$ and 2.10$\sim$2.62$\times$ improvement at 16-bit and 8-bit precision, respectively. 
Energy efficiency also sees notable improvements, with SPEED achieving 1.35$\sim$4.41$\times$ and 1.58$\sim$5.91$\times$ enhancements in contrast with Ara and Yun, respectively.}
% By accommodating multi-precision requirements, SPEED demonstrates its adaptability and versatility in handling a wide range of neural network architectures.
% Compared to some emerging works, such as Dustin\cite{Garofalo2021ESSCIRC} and Darkside\cite{Garofalo2023DARKSIDEAH}, SPEED exhibits a performance gain of up to 5.7$\times$, especially in scenarios where 4-bit is utilized. 
\WX{Compared} to Quark~\cite{Askarihemmat2023QuarkAI}, SPEED exhibits a gain of up to 2.91$\times$, 4.03$\times$, and 1.31$\times$ under 8-bit precision regarding throughput, area efficiency, and energy efficiency, respectively.
% This improvement is a testament to the efficiency and optimization of SPEED's hardware design and dataflow strategies. The ability to achieve superior performance with multi-precision further highlights SPEED's efficiency in executing computationally intensive tasks.
Compared to the Sparq~\cite{Theo2023sparq}, SPEED shows significant throughput improvements, with speedups of up to 3.11$\times$ under 16-bit precision and 11.68$\times$ under 4-bit precision, respectively.
Moreover, SPEED enables efficient 16-bit and 4-bit precision inference that surpasses the best of Sparq by 1.65$\times$ and 6.23$\times$, respectively, on area efficiency. 
In terms of energy efficiency, SPEED also demonstrates an enhancement of 3.55$\times$ for 4-bit precision.
% In summary, SPEED demonstrates a significant throughput improvement, with speedups of 3.11$\sim$6.07$\times$ and 2.91$\sim$7.11$\times$ over existing RISC-V processors \cite{Cavalcante2022NewAra, Perotti2023Yun, Askarihemmat2023QuarkAI, Theo2023sparq} at 16-bit and 8-bit precision conditions,
% and SPEED achieves 1.47$\sim$2.24$\times$ and 2.10$\sim$4.03$\times$ area efficiency improvements under 16-bit and 8-bit precision conditions, respectively,
% % showing its superior area efficiency in multi-precision DNN inference.
% showing its superior throughput in MP-DNN inference under constrained area conditions.
\jOneFC{In summary, SPEED significantly outperforms existing RISC-V processors~\cite{Cavalcante2022NewAra, Perotti2023Yun, Askarihemmat2023QuarkAI, Theo2023sparq}, achieving throughput improvements of up to 6.07$\times$ at 16-bit precision and up to 7.11$\times$ at 8-bit precision, respectively.
Additionally, SPEED demonstrates remarkable area efficiency, with enhancements ranging from 1.47$\times$ to 4.03$\times$ for MP-DNN inference under the constrained area conditions typical in edge computing scenarios.}


